Two-stage Robust Energy Storage Planning with Probabilistic Guarantees: A Data-driven Approach

This paper addresses a central challenge of jointly considering shorter-term (e.g. hourly) and longer-term (e.g. yearly) uncertainties in power system planning with increasing penetration of renewable and storage resources. In conventional planning decision making, shorter-term (e.g., hourly) variations are not explicitly accounted for. However, given the deepening penetration of variable resources, it is becoming imperative to consider such shorter-term variation in the longer-term planning exercise. By leveraging the abundant amount of operational observation data, we propose a scenario-based robust planning framework that provides rigorous guarantees on the future operation risk of planning decisions considering a broad range of operational conditions, such as renewable generation fluctuations and load variations. By connecting two-stage robust optimization with the scenario approach theory, we show that with a carefully chosen number of scenarios, the operational risk level of the robust solution can be adaptive to the risk preference set by planners. The theoretical guarantees hold true for any distributions, and the proposed approach is scalable towards real-world power grids. Furthermore, the column-and-constraint generation algorithm is used to solve the two-stage robust planning problem and tighten theoretical guarantees. We substantiate this framework through a planning problem of energy storage in a power grid with deep renewable penetration. Case studies are performed on large-scale test systems (modified IEEE 118-bus system) to illustrate the theoretical bounds as well as the scalability of proposed algorithm.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> abstract.tex <==
\begin{abstract}
This paper addresses a central challenge in power system planning with increasing penetration of renewable and storage resources. Conventionally shorter-term (e.g., hourly) variations are not explicitly accounted for in the planning exercise in power system, however, given the deepening penetration of variable resources, it is becoming imperative to consider such shorter-term variation in the longer-term planning decision making. 
By leveraging the abundant amount of operational data, we propose a  scenario-based power system robust planning framework that provides rigorous guarantees on the future operation risk of planning decisions considering a broad range of operational conditions, such as  renewable fluctuations and  load variations.
By connecting two-stage robust optimization with the scenario approach theory, we show that with a carefully chosen number of operational scenarios, the operation risk level of the robust solution can be adaptive to risk preferences. The theoretical guarantees hold for any distributions, and the proposed approach is scalable towards real-world systems. Furthermore, the column-and-constraint generation algorithm is used to solve the two-stage robust planning problem and tighten theoretical guarantees. We illustrate the proposed framework on the storage planning problem, which optimizes the siting and sizing of energy storage systems to facilitate the integration of uncertain renewables and loads. This framework can fully  consider the  flexibility value of storage in the power system planning problem. 
Case studies are performed on large-scale test systems (modified IEEE 118-bus system) to verify the theoretical guarantees and illustrate the scalability of the approach.
\end{abstract}

==> ieee-front-matter.tex <==

% paper title
% Titles are generally capitalized except for words such as a, an, and, as,
% at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% not capitalized unless they are the first or last word of the title.
% Linebreaks \\ can be used within to get better formatting as desired.
% Do not put math or special symbols in the title.
\title{Two-stage Risk Adaptable Storage Planning with Probabilistic Guarantees via the Scenario Approach}
%
%
% author names and IEEE memberships
% note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% a structure at a ~ so this keeps an author's name from being broken across
% two lines.
% use \thanks{} to gain access to the first footnote area
% a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% was not built to handle multiple paragraphs
%

\author{
Chao~Yan,~\IEEEmembership{Student~Member,~IEEE},
Xinbo~Geng,~\IEEEmembership{Member,~IEEE},
~Zhaohong~Bie,~\IEEEmembership{Senior~Member,~IEEE},
and~Le~Xie,~\IEEEmembership{Senior~Member,~IEEE}
% <-this % stops a space
\thanks{C. Yan and Z. Bie were with the Department
of Electrical  Engineering, Xi'an Jiaotong University, Xi'an, China, 710049. Emails: yanchao19911224@stu.xjtu.edu.cn and zhbie@xjtu.edu.cn.
X. Geng and L. Xie were with the Department
of Electrical and Computer Engineering, Texas A\&M University, College Station, TX, 77840. E-mails: \{xbgeng,le.xie\}@tamu.edu. Suggested Correspondence: Le Xie.  The work of X. G. is supported in part by NSF CCF-1934904.
\ifx\version\arxiv
C. Yan and X. Geng contributed equally to this paper. C. Yan was in charge of numerical simulations and part of theoretical analysis. X. Geng contributed mainly to the theoretical analysis and paper writing.
\fi
}% <-this % stops a space
}

% note the % following the last \IEEEmembership and also \thanks - 
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
% 
% \author{\cdots.lastname \thanks{\cdots} \thanks{\cdots} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.



% The paper headers
% \markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
% {Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Communications Society Journals}
% The only time the second header will appear is for the odd numbered pages
% after the title page when using the twoside option.
% 
% *** Note that you probably will NOT want to include the author's ***
% *** name in the headers of peer review papers.                   ***
% You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% you desire.




% If you want to put a publisher's ID mark on the page you can do it like
% this:
%\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.



% use for special paper notices
%\IEEEspecialpapernotice{(Invited Paper)}
% make the title area
\maketitle

% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\input{abstract}

% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Power system planning, energy storage, robust optimization, the scenario approach, column-and-constraint generation, short-term uncertainty, operation risk.
\end{IEEEkeywords}

% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

==> temp.tex <==

\section{Introduction}
Power system planning optimizes future investments in the generation, transmission, and storage infrastructures to ensure a reliable, sustainable, and cost-efficient electricity supply meeting future demand \cite{planning_book}. Power system planning is a decision making problem under uncertainties by nature. Traditionally, it mainly deals with \emph{long-term} uncertainties from load growth, fuel price and policies. However, this task becomes particularly challenging due to the growing \emph{short-term} uncertainties from both demand and supply sides \cite{planning_review_2017} such as renewable fluctuations and load variations. Recently, the rapidly growing renewables make it necessary that accurately assessing the flexibility requirements for these short-term operation uncertainties in the long-term planning problem.  To tackle those challenges, two widely-accepted approaches, stochastic optimization (SO) and robust optimization (RO), were adopted for power system planning approaches.

Stochastic optimization often relies on probabilistic description of underlying uncertainties, sampling algorithms are commonly used to approximate the expectation when solving a stochastic program. 
In the context of power system planning, \emph{stochastic} planning approach minimizes the expected cost among many scenarios \cite{transmission_wind,trans_sequential_planning,trans_planning_load_wind,fully_renewable_energy}. In practice, however, probability distribution is only a proxy of uncertainties in the reality and inaccessible in most cases. When solving stochastic planning problems, a large number of scenarios or samples from distributions are required, which causes computational burden when solving real-world scale problems. 

Robust optimization, on the other hand, usually relies on a set-based (often deterministic) modeling of uncertainties. \emph{Robust} planning approach optimizes the expansion and operation costs of the worst-case scenario in a pre-defined uncertainty set. Common choices of uncertainty sets include intervals \cite{interval_minimum_load} and polyhedral uncertainty sets \cite{robust_transmission_planning}. Robust optimization is often scrutinized for returning overly conservative solutions. However, the issue of conservativeness is typically caused by causal choices of uncertainty sets. A good solution to resolve this issue is to construct uncertainty sets using data.

In the context of power system planning, some recent studies pay special attention to short-term operational uncertainties. For example, \cite{stochastic_robust_planning}  used representative scenarios to model short-term operational uncertainties in the robust planning model; \cite{operational_robust_planning} constructed polyhedral uncertainty sets among representative days through clustering historical operational data of a whole year  to represent a wider range of operational conditions. In addition, it models the short-term uncertainties in a daily operational condition not a operational point. This way can consider more temporal dynamics. Once recent publication \cite{adaptive_robust_2020} proposed an adaptive uncertainty set to consider the operational risk of wind fluctuation in the robust planning model. As it aims at the transmission planning problem, it uses an operational point to represent the short-term uncertainty and neglects temporally correlated operating constraints.

In this paper, we demonstrate that a simple construction of uncertainty sets, i.e., the collection of a carefully chosen number of i.i.d. operational scenarios, could resolve this issue. By tuning a risk parameter (violation probability $\epsilon$) and the associated number of scenarios ($K$), planning decisions can be adapted to risk preferences. Meanwhile, the scenarios can be daily operational conditions considering the temporal details. This simple construction of uncertainty set is closely related with the scenario approach theory \cite{campi_exact_2008,calafiore_random_2010,campi_wait-and-judge_2016,campi_general_2018}. The scenario approach has been successfully applied to many power system problems, e.g., resource adequacy and security assessment \cite{reserve_security_framework}, economic dispatch \cite{scenario_dispatch}, demand response scheduling \cite{scenario_demand_response}, and unit commitment \cite{scenario_unit,geng_computing_2019}.

The main advantages of the scenario approach are its \emph{simplicity}, \emph{generality} and \emph{distribution-free} property. The scenario approach theory is based on a simple idea: finding the most cost-efficient solution that is feasible to a set of scenarios. The scenario approach is applicable to \emph{any} convex problem without introducing any additional complexity \cite{bertsimas_tractable_2006}, and becomes one of the most general methods \cite{ben-tal_robust_2009}. The scenario approach is a simple yet rigorous approach. It is a \emph{purely data-driven} approach without constraining on any specific distribution. All theoretical results hold for any distribution \cite{campi_exact_2008,calafiore_random_2010,campi_wait-and-judge_2016,campi_general_2018}.

Nonetheless, the scenario approach was seldom applied in power system planning due to the following reasons: (1) the scenario approach was designed for single-stage optimization problems (no recourse variables), while power system planning is multi-stage ny nature; (2) the discrete decision variables in planning problems cause non-convex formulation, while the classical scenario approach \cite{campi_exact_2008,calafiore_random_2010,campi_wait-and-judge_2016} is only applicable on convex problems; (3) the number of scenarios required by \cite{campi_exact_2008,calafiore_random_2010} grows with the number of decision variables, while power system planning is typically a large-scale optimization problem, the massive amount of scenarios required renders the scenario approach impractical for power system planning.

To the best of our knowledge, references \cite{yang_hybrid_2013,yang_joint_2014,yan_scenario-based_2019} are the only ones that applied the scenario approach on power system planning. The planning problems in \cite{yang_hybrid_2013,yang_joint_2014,yan_scenario-based_2019} were formulated as convex problems to use the classical scenario approach theory \cite{campi_exact_2008,calafiore_random_2010,campi_wait-and-judge_2016}. No binary variables such as optimal locations of renewnables or storages were considered. Furthermore, many technical questions (e.g., if the scenario approach can be applied on multi-stage optimization problems) remain unanswered in the aforementioned references.
Some preliminary results of this paper were reported in \cite{yan_scenario-based_2019}. This paper studies several different formulations of storage planning, and significantly improves \cite{yan_scenario-based_2019} by analyzing both convex and non-convex formulations and providing numerical results on larger-scale systems.

% \XG{say something about the benefits of having theoretical guarantees. Most of references evaluate the planning solution by Monte-Carlo simulations, which rely on a large set of scenarios. Howevever, such an amount of data is not available in practice. Some other approaches have been proposed to verify the planning results: \cite{trans_planning_load_wind} accesses the solution quality of a two-stage stochastic optimization based transmission planning model through obtaining the confidence interval (CI) of the solution in an a-posterior manner. It resorts to a multi-step Monte Carlo simulation based on the stochastic optimization theory  \cite{assess_solution_quality}. For the robust planning model \cite{ROBUST_NETWORK}, it accesses the constraints violation probability of the storage planning solution with a confidence interval through a-posteriori Monte Carlo simulation approach. \cite{robust_transmission_storage_planning} assesses the robustness of the planning solution through a post-optimization approach which calculates the probability of load shedding. [xx] solves the power system planning problem with a reliability index guarantees through a combination of Monte Carlo simulation   and Benders decomposition method. }

The main contributions of this paper are threefold.

(1) We formulate a two-stage robust storage planning problem and solve it using a data-driven approach. Distribution-free theoretical guarantees are provided for both convex and non-convex models on the underlying operation risk of planning decisions for future short-term uncertainties. We also show that the risk of planning decisions consists of two parts:  (a) future operation cost greater than the estimated cost in the planning problem and (b)  the curtailment of load.

(2) Although the scenario approach is commonly used for single-stage decision making, we establish the connection between two-stage RO and the scenario approach theory; the theoretical guarantees of the proposed planning framework are obtained via this connection by examining the cardinality of invariant sets\footnote{The set of support scenarios if using the term in the original theory \cite{campi_exact_2008}.}. We show that the cardinality of minimal invariant sets of convex or non-convex two-stage robust storage planning (RSP)  problems is often small, regardless of problem size or power system scale. For large systems, we can achieve the same risk level using a moderate number of scenarios, thus the proposed approach is very scalable.

(3) The two-stage robust storage planning problem is solved via the column-and-constraint generation algorithm, we further show that C\&CG algorithm could find invariant set numerically thus improve the theoretical guarantees. Finally, we want to emphasize that the proposed approach is a general framework and many results in this paper still hold for general power system planning problems.

(4) \XG{a real case study, improvement in reducing the number of scenarios, computation time, guarantees. intuitions for power engineers}

The notations in this paper are standard. All matrices and vectors are in the real field $\mathbb{R}$.
% We use $\bm{1}$ to represent an all-one vector of appropriate size, and $\bm{0}$ to denote an all-zero vector or the origin.
Matrices and vectors are in bold fonts, e.g., $\bm{A}$ and $\bm{b}$. The transpose of a vector $\bm{a}$ is $\bm{a}^\intercal$, and the $j$th entry of vector $\bm{a}$ is $a_j$. 
Sets are in calligraphy fonts, e.g. the set of transmission lines $\mathcal{L}$. The cardinality of a set $\mathcal{S}$ is $|\mathcal{S}|$.
Related variables are represented by the same letter but distinct superscripts. For instance, $p_{l,t}^{\mathcal{L}}$ denotes the line flows, and $p_{i,n,t}^{\mathcal{G}}$ is the generation output.
The upper and lower bounds on variable $\bm{a}$ are denoted by $\overline{\bm{a}}$ and $\underline{\bm{a}}$, respectively. All proofs and detailed algorithms are provided in the appendix.

The remainder of this paper is organized as follows. Section \ref{sec:background} first introduces two-stage robust optimization and C\&CG algorithm, then connects them with the scenario approach theory and provides key theoretical results. Section \ref{sec:storage_planning} formulates the two-stage robust storage planning problem, based on the theorems in Section \ref{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach}, Section \ref{sec:theoretical_analysis} provides theoretical guarantees on operation risk of the optimal storage planning results. Section \ref{sec:case_study} presents numerical results.
Concluding remarks and future works are in Section \ref{sec:concluding_remarks}.
% Additional discussions and concluding remarks are in Section \ref{sec:discussions} and Section \ref{sec:concluding_remarks}.

\section{Background} % (fold)
\label{sec:background}
% Section \ref{sub:two_stage_robust_optimization} and \ref{sub:column_and_constraint_generation_algorithm} introc
% This section first introduces two-stage robust optimization and how to solve it using the column-and-constraint generation (C\&CG) algorithm. Section \ref{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach} demonstrates the feasibility guarantees on the optimal solution, and shows that how the C\&CG algorithm could assist to obtain the theoretical guarantees.

\subsection{Two-stage Robust Optimization} % (fold)
\label{sub:two_stage_robust_optimization}
A standard two-stage robust optimization problem is \eqref{opt:two-stage-robust}.
\begin{equation}
\label{opt:two-stage-robust}
\min _{\bm{x} \in \mathcal{X} } \left(\bm{c}^{\intercal} \bm{x}+ \max _{\bm{\delta} \in \bm{\Delta}} \min _{\bm{y} \in \mathcal{Y}(\bm{x}; \bm{\delta})} \bm{d}^{\intercal} \bm{y}\right)
\end{equation}
It seeks the objective-minimizing solution $(\bm{x}^*, \bm{y}^*)$ for the worst scenario $\bm{\delta} \in \Delta$ in a pre-defined \emph{uncertainty set} $\Delta$. Without loss of generality (see Appendix \ref{ssub:epigraph_formulation}), we assume deterministic objectives, i.e., no randomness asscociated with $\bm{c}$ and $\bm{d}$. Sets $\mathcal{X} \subseteq \mathbb{R}^{n_x}$ and $\mathcal{Y} \subseteq \mathbb{R}^{n_y}$ denote the constraints for the first and second stages, respectively.
Note that the second stage constraint $\mathcal{Y}(\bm{x}; \bm{\delta})$ is determined by the first stage decision $\bm{x}$ and uncertainty $\bm{\delta}$. We follow the convention that $\bm{d}^{\intercal} \bm{y} = +\infty$ if the second-stage problem $ \min_{\bm{y} \in \mathcal{Y}(\bm{x}; \bm{\delta})} \bm{d}^{\intercal} \bm{y}$ is infeasible. We say that a solution is feasible to \eqref{opt:two-stage-robust} if it has a finite objective value.
\begin{defn}[Feasible Solution]
We say $(\bm{x},\bm{y})$ is a \emph{feasible solution} to \eqref{opt:two-stage-robust} if (i) $\bm{x} \in \mathcal{X}$; and (ii) $\bm{y} \in \mathcal{Y}(\bm{x}; \bm{\delta})$ for all $\bm{\delta} \in \Delta$.
\end{defn}
Problem \eqref{opt:two-stage-robust} is often solved to find the the \emph{optimal solution} $(\bm{x}^*,\bm{y}^*)$ to \eqref{opt:two-stage-robust}. Similar with standard optimization problems, we say that $(\bm{x}^*, \bm{y}^*)$ is an (globally) \emph{optimal solution} to \eqref{opt:two-stage-robust}, if $\bm{c}^\intercal \bm{x}^* + \bm{d}^\intercal \bm{y}^* \le \bm{c}^\intercal \bm{x}^\diamond + \bm{d}^\intercal \bm{y}^\diamond$ for all feasible solution $(\bm{x}^\diamond, \bm{y}^\diamond)$ to \eqref{opt:two-stage-robust}.
\begin{rem}[Infeasible Solution]
\label{rem:infeasible_solution}
For any potentially better solution $(\bm{x}^\diamond, \bm{y}^\diamond)$ with $\bm{c}^\intercal \bm{x}^\diamond + \bm{d}^\intercal \bm{y}^\diamond < \bm{c}^\intercal \bm{x}^* + \bm{d}^\intercal \bm{y}^*$, there always exists a $\bm{\delta}^\diamond \in \Delta$ such that $(\bm{x}^\diamond, \bm{y}^\diamond)$ is infeasible, i.e., $\bm{y}^\diamond \notin \mathcal{Y}(\bm{x}^\diamond; \bm{\delta}^\diamond)$.
\end{rem}

% \begin{prop}
% \label{prop:worst_case_solution_is_optimal}
% Let $(\bm{x}^*, \bm{y}^*)$ and $\bm{\delta}^*$ denote the optimal solution and worst scenario to \eqref{opt:two-stage-robust}. Suppose $(\bm{x}^\star,\bm{y}^\star)$ is the optimal solution to \eqref{opt:two-stage-given-scenario} with $\bm{\delta}^\diamond = \bm{\delta}^*$, then $\bm{c}^\intercal \bm{x}^\star + \bm{d}^\intercal \bm{y}^\star = \bm{c}^\intercal \bm{x}^* + \bm{d}^\intercal \bm{y}^*$.
% \end{prop}
% This claim is problematic

% \begin{proof}[Proof of Proposition \ref{prop:worst_case_solution_is_optimal}]
% (i) If $\bm{c}^\intercal \bm{x}^\star + \bm{d}^\intercal \bm{y}^\star > \bm{c}^\intercal \bm{x}^* + \bm{d}^\intercal \bm{y}^*$, then $(\bm{x}^*, \bm{y}^*)$ is feasible to \eqref{opt:two-stage-given-scenario} with smaller objective than $(\bm{x}^\star,\bm{y}^\star)$, which clearly is a contradiction. (ii) If $\bm{c}^\intercal \bm{x}^\star + \bm{d}^\intercal \bm{y}^\star < \bm{c}^\intercal \bm{x}^* + \bm{d}^\intercal \bm{y}^*$, Remark \ref{rem:infeasible_solution} tells us there exists 
% \end{proof}

In this paper, we only consider the case in which all constraints are linear.
\begin{subequations}
\begin{align}
\mathcal{X} &:=\{\bm{x} \in \mathbb{R}^{n_x}: {\bm{A}\bm{x} \le \bm{b}} \}\\
\mathcal{Y}(\bm{x}; \bm{\delta}) &:= \left\{\bm{y} \in \mathbb{R}^{n_y}: \bm{G} \bm{y} \le \bm{h},  \bm{T}(\bm{\delta}) \bm{x} + \bm{Q}(\bm{\delta}) \bm{y} \le  \bm{r}(\delta) \right\}
\end{align}
\end{subequations}
Matrix $\bm{Q}(\bm{\delta})$ is the \emph{recourse} matrix.
Throughout this paper, we focus on the cases where the second-stage problem is feasible, which is formally defined as \emph{relatively complete recourse}. This is mainly for the purpose of simplifying theorems and algorithms. Most results in Sections \ref{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach} and \ref{sec:theoretical_analysis} can be easily generalized towards situations \emph{without} relatively complete recourse. Detailed discussions in different contexts are provided accordingly.
\begin{defn}[Relatively Complete Recourse \cite{zeng2013solving}]
\label{def:relative}
% \eqref{opt:two-stage-robust} is said to have \emph{fixed recourse} if $\bm{Q}(\bm{\delta})$ is not subject to uncertainty, i.e., $\bm{Q}(\bm{\delta}) = \bm{Q}$.
Two-stage RO problem \eqref{opt:two-stage-robust} is said to have \emph{relatively complete recourse}, if for any $\bm{x} \in \mathcal{X}$ and $\bm{\delta} \in \Delta$, the second stage problem $\min _{\bm{y} \in \mathcal{Y}(\bm{x}; \bm{\delta})} \bm{d}^{\intercal} \bm{y}$ is feasible, i.e., $\mathcal{Y}(\bm{x}; \bm{\delta}) \ne \emptyset$.
\end{defn}
One critical observation is that \eqref{opt:two-stage-robust} can be formulated as a \emph{single-stage} robust problem\footnote{This observation may not be true for adjustable robust optimization problems, see Chapter 14 of \cite{ben-tal_robust_2009} and Section 6 of \cite{gorissen_practical_2015} for in-depth discussions.}. The following proposition lays the foundation of the main theoretical results (Theorems \ref{thm:apriori_guarantee_convex}, \ref{thm:aposteriori_guarantee_convex} and \ref{thm:aposteriori_guarantee_nonconvex}) of this paper.
\begin{prop}
\label{prop:two-stage-RO-as-one-stage}
% Suppose $\Delta$ is compact, and $\mathcal{Y}(\bm{x}; \bm{\delta})$ is compact for every $\bm{x} \in \mathcal{X}$ and $\bm{\delta} \in \Delta$.
The two-stage robust optimization problem \eqref{opt:two-stage-robust} is \emph{equivalent} to the single-stage problem \eqref{opt:two-stage-robust-single}:
\begin{subequations}
\label{opt:two-stage-robust-single}
\begin{align}
\min_{\bm{x} \in \mathcal{X},\gamma}~&\bm{c}^{\intercal} \bm{x} + \gamma \\
\text{s.t.}~& (\bm{x},\gamma) \in \mathcal{Z}(\bm{\delta}) ,~\forall \bm{\delta} \in \Delta.
\end{align}
\end{subequations}
in which $\mathcal{Z}(\bm{\delta}) := \{(\bm{x},\gamma): \exists \bm{y} \in \mathcal{Y}(\bm{x}; \bm{\delta})~\text{and}~\bm{d}^{\intercal} \bm{y} \le \gamma\}$.
We say \eqref{opt:two-stage-robust} is equivalent with \eqref{opt:two-stage-robust-single} in the sense that they share the same (globally) optimal first-stage solutions and optimal objective values.
\end{prop}
%More specifically, (i) if $(\bm{x}^*,\bm{y}^*, \bm{\delta}^*)$ is an optimal solution \eqref{opt:two-stage-robust}, then there exists a $\gamma^*$ such that $(\bm{x}^*,\bm{\gamma}^*)$ is optimal to \eqref{opt:two-stage-robust-single}; (ii) if $(\bm{x}^\star,\bm{\gamma}^\star)$ is an optimal solution to \eqref{opt:two-stage-robust-single}, then there exists a $(\bm{y}^\star, \bm{\delta}^\star)$ such that $(\bm{x}^\star,\bm{y}^\star, \bm{\delta}^\star)$ is optimal to \eqref{opt:two-stage-robust}.

The seemingly simple formulation \eqref{opt:two-stage-robust-single} may not be solved directly, the main reason is that set $\mathcal{Z}(\bm{\delta})$ could be complicated (e.g., the intersection of an exponential number of half-spaces), sometimes an analytical form of $\mathcal{Z}(\bm{\delta})$ may not even exist. Proposition \ref{prop:two-stage-RO-as-one-stage} only aims at connecting two-stage RO problems with the single-stage scenario approach theory in Section \ref{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach}.
% For computational studies, we solve the two-stage formulation \eqref{opt:two-stage-robust} using the column-and-constraint generation algorithm.

In the remainder of this paper, we make the choice that the uncertainty set $\Delta$ is a collection of $K$ i.i.d. realizations of random variables $\bm{\delta}$, i.e., $\Delta = \mathcal{K} := \{\bm{\delta}^{(1)},\bm{\delta}^{(2)},\cdots,\bm{\delta}^{(K)}\}$. In Section \ref{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach}, we show that this simple construction of uncertainty sets possesses rigorous theoretical guarantees. In addition, uncertainty set $\Delta = \mathcal{K}$ does not introduce any additional computational complexity (unlike ellipsoidal or conic uncertainty sets in \cite{bertsimas_tractable_2006}, which sometimes render solving RO problems intractable), and the resulting two-stage RO problem can be efficiently solved by C\&CG algorithm.
% subsection two_{n}tage_robust_optimization (end)

\subsection{Column-and-Constraint Generation (C\&CG) Algorithm} % (fold)
\label{sub:column_and_constraint_generation_algorithm}
% \XG{[A brief overview of available algorithms]}.
One popular algorithm to solve the two-stage RO problem is the column-and-constraint generation (C\&CG) algorithm \cite{zeng2013solving}. When the uncertainty set is a collection of $K$ discrete scenarios $\mathcal{K} := \{\bm{\delta}^{(1)},\bm{\delta}^{(2)},\cdots,\bm{\delta}^{(K)}\}$,
\begin{equation}
\label{opt:two-stage-robust-scenarios}
\min _{\bm{x} \in \mathcal{X} } \left(\bm{c}^{\intercal} \bm{x}+ \max _{\bm{\delta} \in \mathcal{K} } \min _{\bm{y} \in \mathcal{Y}(\bm{x}; \bm{\delta})} \bm{d}^{\intercal} \bm{y}\right)
\end{equation}
Proposition \ref{prop:two-stage-RO-as-one-stage} shows that \eqref{opt:two-stage-robust-scenarios} is equivalent with 
\begin{subequations}
\label{opt:two-stage-robust-single-scenario}
\begin{align}
\min_{\bm{x},\gamma}~&\bm{c}^{\intercal} \bm{x} + \gamma \\
\text{s.t.}~& \bm{x} \in \mathcal{X}~\text{and}~(\bm{x},\gamma) \in \cap_{i=1}^{K} \mathcal{Z}(\bm{\delta}^{(i)}) 
\end{align}
\end{subequations}
Constraint $(\bm{x},\gamma) \in \cap_{i=1}^{K} \mathcal{Z}(\bm{\delta}^{(i)})$ can be explicitly written as \eqref{opt:two-stage-robust-two-scenario} by introducing additional variables $\{\bm{y}^{(1)},\cdots, {\bm{y}^{(K)}}\}$. Variable $\bm{y}^{(k)}$ is the recourse decision variable for the $k$th scenario $\bm{\delta}^{(k)}$.
\begin{subequations}
\label{opt:two-stage-robust-two-scenario}
\begin{align}
% \min _{\bm{x},\gamma,\bm{y}^{(1)},\cdots,\bm{y}^{(K)} }~ &\bm{c}^{\intercal} \bm{x}+ \gamma\\
% \text{s.t.}~&\bm{x} \in \mathcal{X}\\ 
&\bm{d}^{\intercal} \bm{y}^{(k)} \le \gamma,~k=1,2,\cdots,K. \\
& \bm{y}^{(k)}\in \mathcal{Y}(\bm{x}, \bm{\delta}^{(k)}),~k=1,2,\cdots,K.
\end{align}
\end{subequations}
Therefore, solving the two-stage RO problem \eqref{opt:two-stage-robust} is equivalent to solve a single-stage optimization problem. It is worth pointing out that constraint \eqref{opt:two-stage-robust-two-scenario} is simply enumerating \emph{all} $K$ scenarios. When seeking risk-averse solutions, which is common for power system applications, the number of scenarios $K$ could be colossal. Thus \eqref{opt:two-stage-robust-two-scenario} consists of a gigantic number of decision variables and constraints, which is extremely inefficient or even impossible to solve. A \emph{partial} enumeration such as the C\&CG algorithm in Section \ref{sub:column_and_constraint_generation_algorithm} could significantly outperform the approach of solving \eqref{opt:two-stage-robust-two-scenario} in one shot.
 % (solving the problem much faster and uses less memory).

The intuition behind the C\&CG algorithm is quite simple: only a small portion $\mathcal{O}$ of the uncertainty set $\Delta$ matters, e.g., extreme points of $\Delta$ along the optimization direction. C\&CG algorithm is essentially an iterative procedure to identify critical scenarios $\mathcal{O}$. The C\&CG algorithm iteratively adds constraints $(\bm{x},\gamma) \in \cap_{i \in \mathcal{O}} \mathcal{Z}(\bm{\delta}^{(l)})$ to the problem (\emph{constraint generation}). Since constraint $(\bm{x},\gamma) \in \mathcal{Z}(\bm{\delta}^{(l)})$ guarantees the existence of feasible recourse variable $\bm{y}^{(l)} \in \mathcal{Y}(\bm{x}; \bm{\delta})$, additional second-stage variables are introduced (\emph{column generation}).
Algorithm \ref{alg:CCG} in Appendix \ref{sub:algorithms} formally defines the C\&CG algorithm. More details and theoretical analysis on C\&CG can be found in \cite{zeng2013solving}.
% subsection column_and_constraint_generation_algorithm (end)

\subsection{Probabilistic Guarantees via the Scenario Approach} % (fold)
\label{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach}
Throughout this paper, we construct the uncertainty set $\Delta$ using $K$ i.i.d. scenarios $\Delta = \mathcal{K} := \{\bm{\delta}^{(1)},\bm{\delta}^{(2)},\cdots,\bm{\delta}^{(K)}\}$. The resulting optimization problems are presented in \eqref{opt:two-stage-robust-single-scenario}  and \eqref{opt:two-stage-robust-two-scenario}.
Let $(\bm{x}_{\mathcal{K}}^*,\gamma_{\mathcal{K}}^*)$ denote the optimal solution to \eqref{opt:two-stage-robust-single-scenario}, e.g., returned by the C\&CG algorithm. The main results of the scenario approach theory connects the number of scenarios $K$ with the violation probability of a candidate solution.
\begin{defn}[Violation Probability]
\label{def:violation probability}
The violation probability of a candidate solution $(\bm{x}^\diamond,\gamma^\diamond)$ to \eqref{opt:two-stage-robust-single-scenario} is defined as
\begin{equation}
\mathbb{V}(\bm{x}^\diamond, \gamma^\diamond) := \mathbb{P}_{\bm{\delta}}\big( (\bm{x}^\diamond, \gamma^\diamond) \notin \mathcal{Z}(\bm{\delta}) \big)
\end{equation}
\end{defn}
\begin{rem}
\label{rem:violation_probability_interpretation_general}
The violation probability $\mathbb{V}(\bm{x}_{\mathcal{K}}^*,\gamma_{\mathcal{K}}^*)$ quantifies the quality of the robust solution $(\bm{x}_{\mathcal{K}}^*,\gamma_{\mathcal{K}}^*)$. In other words, $\mathbb{V}(\bm{x}_{\mathcal{K}}^*,\gamma_{\mathcal{K}}^*)$ is the probability that the following two events happen: (i) $\mathcal{Y}(\bm{x}_{\mathcal{K}}^*; \bm{\delta})$ is empty (infeasible second-stage problem); or (ii) there exists a feasible $\bm{y} \in \mathcal{Y}(\bm{x}_{\mathcal{K}}^*; \bm{\delta})$ but $\bm{d}^{\intercal} \bm{y} > \gamma_{\mathcal{K}}^*$.
\end{rem}
The main theorems of the scenario approach theory are based on the key definitions of invariant set and essential set\footnote{For the convex case in Theorem \ref{thm:apriori_guarantee_convex}, \cite{geng_computing_2019} shows that the essential set is the set of support scenarios as in \cite{campi_exact_2008}. For non-convex case, an essential set is the minimal support-subsample in \cite{campi_general_2018}.}. 

\begin{defn}[Invariant Set $\mathcal{I}$ and Essential Set $\mathcal{E}$]
Let $(\bm{x}_{\mathcal{I}}^*,\gamma_{\mathcal{I}}^*)$ denote the optimal solution to \eqref{opt:two-stage-robust-single-scenario} using a subset of scenarios $\mathcal{I} \subseteq \mathcal{K}$. Set $\mathcal{I}$ is an Invariant Set if $\bm{c}^{\intercal} \bm{x}_{\mathcal{I}}^* + \gamma_{\mathcal{I}}^* = \bm{c}^{\intercal} \bm{x}_{\mathcal{K}}^* + \gamma_{\mathcal{K}}^*$. The invariant set with the smallest cardinality is the Essential Set $\mathcal{E}$.
\end{defn}

The original scenario approach theory \cite{campi_exact_2008,campi_wait-and-judge_2016,campi_general_2018,geng_computing_2019} only applies to single-stage optimization problems. There is a lack of known results  of multi-stage scenario approach. 
Proposition \ref{prop:two-stage-RO-as-one-stage} shows that the two-stage robust optimization problem has an equivalent single-stage formulation. We extend the classical scenario approach theory towards two-stage decision making problems.
Theorems \ref{thm:apriori_guarantee_convex}, \ref{thm:aposteriori_guarantee_convex} and \ref{thm:aposteriori_guarantee_nonconvex} provide guarantees on the risk of the robust solution $(\bm{x}_{\mathcal{K}}^*,\gamma_{\mathcal{K}}^*)$. 
After converting the scenario-based two-stage robust optimization as the single-stage scenario program, Theorem \ref{thm:apriori_guarantee_convex} is essentially Theorem 1 of \cite{campi_exact_2008}, Theorem \ref{thm:aposteriori_guarantee_convex} is from Theorem 2 of \cite{campi_wait-and-judge_2016}, and Theorem \ref{thm:aposteriori_guarantee_nonconvex} is a direct corollary of Theorem 1 in \cite{campi_general_2018}. The relatively completely recourse assumption is necessary to meet the feasibility assumption in \cite{campi_exact_2008,campi_wait-and-judge_2016,campi_general_2018,geng_computing_2019} (see Assumption \ref{ass:feasibility} in Appendix \ref{sub:single_stage_decision_making}).
\begin{thm}[Prior Guarantees \cite{campi_exact_2008}]
\label{thm:apriori_guarantee_convex}
Suppose \eqref{opt:two-stage-robust-scenarios} is convex and has relatively complete recourse.
Given an acceptable risk level $\epsilon \in (0,1)$, a confidence parameter $\beta \in (0,1)$, and the number of first-stage decision variables $d$ of \eqref{opt:two-stage-robust-single-scenario}. Let $K$ be the smallest integer that
\begin{equation}
\label{eqn:K_choice_convex}
\sum_{i=0}^{d-1} \binom{K}{i} \epsilon^i (1- \epsilon)^{K-i} \le \beta
\end{equation}
then $\mathbb{P}^K\big( \mathbb{V}(\bm{x}_{\mathcal{K}}^*, \gamma^*) > \epsilon \big) \le \beta$, where $(\bm{x}^*, \gamma^*)$ is the optimal solution to \eqref{opt:two-stage-robust-single-scenario} with $K$ i.i.d. scenarios.
\end{thm}

\begin{thm}[Posterior Guarantees for Convex Problems \cite{campi_wait-and-judge_2016}]
\label{thm:aposteriori_guarantee_convex}
Suppose \eqref{opt:two-stage-robust-scenarios} is convex and has relatively complete recourse. 
Given a confidence parameter $\beta \in (0,1)$ and $(\bm{x}_{\mathcal{K}}^*, \gamma^*)$ is the optimal solution to \eqref{opt:two-stage-robust-single-scenario}. Let $|\mathcal{I}|$ be the cardinality of an invariant set, then the following probabilistic guarantee holds:
\begin{equation}
  \mathbb{P}^K \Big(\mathbb{V}(\bm{x}_{\mathcal{K}}^{*}, \gamma^*) \ge \epsilon(|\mathcal{I}|) \Big) \le \beta,
\end{equation}
where $0 < \epsilon(k) < 1$ is the (unique) solution to the polynomial equation given an integer $k=0,1,\cdots,K$,
\begin{equation}
\label{eqn:poster_convex_epsilon_function}
  \frac{\beta}{K+1} \sum_{i=k}^K \binom{i}{k} (1- \epsilon)^{i-k} - \binom{K}{k}(1- \epsilon)^{K-k} = 0
\end{equation}
\end{thm}

\begin{thm}[Probabilistic Guarantees for Non-convex Problems  \cite{campi_general_2018}]
\label{thm:aposteriori_guarantee_nonconvex}
Suppose \eqref{opt:two-stage-robust-scenarios} has relatively complete recourse, and $(\bm{x}_{\mathcal{K}}^*, \gamma^*)$ is the optimal solution to \eqref{opt:two-stage-robust-single-scenario}, let $\mathcal{I}_{\mathcal{K}}$ be an invariant set of \eqref{opt:two-stage-robust-single-scenario} using $K$ scenarios, then the following probabilistic guarantee holds:
\ifx\version\arxiv
\begin{equation}
\label{eqn:sample_complexity_nonconvex_epsilon}
\mathbb{P}^K\big( \mathbb{V}(\bm{x}_{\mathcal{K}}^*, \gamma^*) > \epsilon(|\mathcal{I}_{\mathcal{K}}|, \beta) \big) \le \beta,~\text{where}~\epsilon(k,\beta) := 
  \begin{cases}
  1&~\text{if}~k=K; \\
  1 - \Big( \frac{\beta}{K \binom{K}{k}} \Big)^{\frac{1}{K-k}} &~\text{otherwise}.
  \end{cases}
\end{equation}
\else
\begin{equation}
\label{eqn:sample_complexity_nonconvex_epsilon}
\mathbb{P}^K\big( \mathbb{V}(\bm{x}_{\mathcal{K}}^*, \gamma^*) > \epsilon(|\mathcal{I}_{\mathcal{K}}|, \beta) \big) \le \beta,
\end{equation}
where 
\begin{equation}
\epsilon(k,\beta) := 
  \begin{cases}
  1&~\text{if}~k=K; \\
  1 - \Big( \frac{\beta}{K \binom{K}{k}} \Big)^{\frac{1}{K-k}} &~\text{otherwise}.
  \end{cases}
\end{equation}
\fi
\end{thm}

Although Theorems \ref{thm:apriori_guarantee_convex}, \ref{thm:aposteriori_guarantee_convex} and \ref{thm:aposteriori_guarantee_nonconvex} hold for \emph{any} invariant set, the tightest guarantee is achieved for the essential set, i.e., the invariant set with minimal cardinality \cite{geng_computing_2019}.
In general, finding essential sets is a combinatorial problem, which could be computationally intractable for non-convex scenario problems \eqref{opt:two-stage-robust-scenarios}).
Proposition \ref{prop:CCG_return_invariant_set} shows that C\&CG algorithm can effectively narrow down range of searching.
\begin{prop}
\label{prop:CCG_return_invariant_set}
The set $\mathcal{O}$ returned by Algorithm \ref{alg:CCG} (C\&CG) is an invariant set.
\end{prop}
Proposition \ref{prop:CCG_return_invariant_set} is almost self-evident. The last step of C\&CG is to solve a two-stage RO problem with all scenarios in $\mathcal{O}$. \cite{zeng2013solving} shows that C\&CG algorithm converges to the optimal solution to \eqref{opt:two-stage-robust-two-scenario}. By definition, $\mathcal{O}$ is an invariant set (not necessarily the minimal one). In general, C\&CG algorithm can converge after few iterations so that the cardinality of $\mathcal{O}$ is usually small, then we can use Algorithm \ref{alg:irr} to identify the essential set from $\mathcal{O}$.
% subsection adaptive_robust_optimization (end)

\section{Storage Planning} % (fold)
\label{sec:storage_planning}
Energy storage is a key resource to facilitate the integration of renewable energy resources by providing operational flexibility and ancillary services \cite{xu_scalable_2017}. As of 2019, PJM has deployed approximately 300 MW of energy storage \cite{hsia_energy_2019}; about 20 MW grid-scale battery-storage projects have come on-line at ISO New England since 2015, and nearly 2300 MW of grid-scale stand-alone energy-storage projects are requesting interconnection \cite{iso_new_england_2020_2020}.
Appropriate placements of energy storage systems could maximize the value of storage on the secure and economic operation of power systems. 
Storage planning, which optimizes the siting and sizing of energy storage\cite{storage_size_site,storage_technology}, becomes a topic of increasing importance in power system planning. Similar with other planning problems, various approaches have been proposed to deal with uncertainties, e.g., stochastic storage planning \cite{stochastic_storage_planning}, robust optimization planning \cite{robust_storage_in}, and chance-constrained planning \cite{chance_storage_planning}. Because storage is a resource that provides temporal flexibility, the consideration of temporal operational dynamics of short-term uncertainties is very important for its planning to effectively reduce future operation risk.  

\subsection{Nomenclature} % (fold)
\label{sub:nomenclature}
For notation simplicity, we use $(\cdots)\text{s}$ to denote the collection of variables, e.g., $\{(E_{n}, P_{n}, z_n)\}_{n \in \mathcal{N}}$ is denoted by $(E_{n}, P_{n}, z_n)\text{s}$. Unless specified, all decision variables are continuous variables. For simplicity, we assume that storage systems can be installed at every bus, i.e., $\mathcal{S} = \mathcal{N}$, thus all variables related with storage systems is indexed by the bus index $n$, e.g., $e_{n,t}^{\text{SOC}}$.

\noindent Sets and indices
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$o(l), r(l)$}]
\item[$i,j,k$] indices for general purposes;
\item[$s,t,l,n$] indices for storages, time, lines and nodes
\item[$\mathcal{G}(n)$] the set of generators at bus $n$;
\item[$\mathcal{T}$] the set of time;
\item[$\mathcal{N}$] the set of buses;
\item[$\mathcal{L}$] the set of transmission lines;
\item[$\mathcal{S}$] potential locations of storage systems;
\item[$o(l), r(l)$] sending and receiving nodes of a line, i.e., $l = (o(l),r(l))$;
\item[$\mathcal{W}$] the set of wind farms.
\end{IEEEdescription}
First-stage Variables
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$P_{n}$}]
\item[$E_{n}$] the energy capacity (MWh) of the storage system;
\item[$P_{n}$] the power capacity (MW) of the storage system;
\item[$z_{n}$] integer variables, number of storage units.
\end{IEEEdescription}
Second-stage Variables
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$p_{n,t}^{\text{ch}}, p_{n,t}^{\text{dis}}$}]
\item[$p_{n,t}^{\text{ch}}, p_{n,t}^{\text{dis}}$] the charging and discharging power (MW) of the storage system at node $n$;
\item[$p_{i,n,t}^{\mathcal{G}}$] generator output;
\item[$p_{l,t}^{\mathcal{L}}$] line power flow;
\item[$\theta_{n,t}$] nodal voltage angle;
\item[$e_{n,t}^{\text{SOC}}$] state of charge (SOC) of a storage;
\item[$p_{n,t}^{\text{shed}}$] nodal load shedding/shedding.
\end{IEEEdescription}
Parameters
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$\eta_{n}^{\text{ch}}, \eta_{n}^{\text{dis}}$}]
\item[$C_{n}^{\text{E}}$] annualized storage energy investment cost;
\item[$C_{n}^{\text{P}}$] annualized storage power investment cost;
\item[$c_i^{\mathcal{G}}$] hourly incremental generation cost;
\item[$c_{n}^{\text{dis}}, c_{n}^{\text{ch}}$] hourly incremental discharging/charging cost, related with the degradation cost of storage units;
\item[$c_n^{\text{shed}}$] cost of load shedding;
\item[$\underline{p_i^{\mathcal{G}}}, \overline{p_i^{\mathcal{G}}}$] generator output lower/upper limit;
\item[$\underline{p_l^{\mathcal{L}}}, \overline{p_l^{\mathcal{L}}}$] transmission power flow lower/upper limit;
\item[$\eta_{n}^{\text{ch}}, \eta_{n}^{\text{dis}}$] storage charge/discharge efficiency;
\item[$C^{\text{Budget}}$] storage investment budget;
\item[$x_l$] transmission line reactance;
\item[$\overline{\rho}, \underline{\rho}$] maximum/minimum power/energy ratio;
\item[$\overline{R}_{i}, \underline{R}_{i}$] generator ramp up/down limit;
\item[$K_d$] the weight of operational cost;
\item[$v_{n,t}$] binary variable, indicating charging/discharging status of storage devices;
\item[$q^{E}$] quantized energy capacity;
\item[$q^{P}$] quantized power capacity;
\item[$\overline{w_{n}}$] maximum wind capacity at node $n$;
\item[$\overline{d_{n}}$]  peak load at node $n$.
\end{IEEEdescription}
Uncertainties
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$w_{n,t}$}]
\item[$\bm{\delta}_{s}$] uncertainties in storage planning, $\bm{\delta_{s}} := (\alpha^w_{n,t},\alpha^d_{n,t})\text{s}$;
\item[$\alpha^w_{n,t}$] wind capacity factor at bus $n$ at time $t$;
\item[$\alpha^d_{n,t}$] load factor at bus $n$ at time $t$.
\end{IEEEdescription}

% section nomenclature (end)

\subsection{Deterministic Storage Planning} % (fold)
\label{sub:deterministic_storage_planning}
We first introduce the deterministic storage planning problem \eqref{opt:det-SP}, which is a two-stage optimization problem.
\begin{align}
\min_{ \bm{x} \in \Xi_{1}}~ C(\bm{x}) + K_d \min_{ \bm{y} \in \Xi_{2}(\bm{x}; \bm{\delta})} c(\bm{y})  \label{opt:det-SP} 
\end{align}
\subsubsection{Objective} % (fold)
\label{ssub:objective_DSP}
There are two common storage planning formulations: cost-oriented formulation and curtailment-oriented formulation. They only differ in the objectives.
\paragraph{Cost-Oriented Storage Planning}
The objective of the cost-oriented formulation is \eqref{opt-det:cost}. The \emph{first stage} determines the optimal energy and power capacity $\bm{x} = (E_{n}, P_{n}, z_{n})$ of the storage units at bus $n$ by minimizing total investment cost \eqref{opt-det:planning-obj-cost}. 
The \emph{second stage} optimizes the daily operation cost \eqref{opt-det:operation-obj-2} of the planned storages $(p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}})$, generation $p_{i,n,t}^{\mathcal{G}}$, and load shedding $p_{n,t}^\text{shed}$, i.e., $\bm{y} = (p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}},p_{i,n,t}^{\mathcal{G}},p_{n,t}^\text{shed},v_{n,t})$. 

\ifx\version\arxiv 
\begin{subequations}
\label{opt-det:cost}
\begin{align}
& C(\bm{x}) := \sum_{n\in \mathcal{N}} (C_{n}^{\text{E}} E_{n} +  C_{n}^{\text{P}} P_{n}) \label{opt-det:planning-obj-cost} \\
& c(\bm{y}) := \sum_{t\in \mathcal{T}} \sum_{n \in \mathcal{N}}  \sum_{i\in \mathcal{G}(n)} c_{i,n}^{\mathcal{G}} p_{i,n,t}^{\mathcal{G}} + \sum_{t\in \mathcal{T}}  \sum_{n\in \mathcal{N}} (c_{n}^\text{ch} p_{n,t}^{\text{ch}}  +c_{n}^\text{dis} p_{n,t}^{\text{dis}}) +\sum_{t\in \mathcal{T}}  \sum_{n\in \mathcal{N}} c_{n}^\text{shed} p_{n,t}^\text{shed} \label{opt-det:operation-obj-2}
\end{align}
\end{subequations}
\else
\begin{subequations}
\label{opt-det:cost}
\begin{align}
& C(\bm{x}) := \sum_{n\in \mathcal{N}} (C_{n}^{\text{E}} E_{n} +  C_{n}^{\text{P}} P_{n}) \label{opt-det:planning-obj-cost} \\
& c(\bm{y}) := \sum_{t\in \mathcal{T}} \sum_{n \in \mathcal{N}}  \sum_{i\in \mathcal{G}(n)} c_{i,n}^{\mathcal{G}} p_{i,n,t}^{\mathcal{G}} + \sum_{t\in \mathcal{T}} \sum_{n\in \mathcal{N}} (c_{n}^\text{ch} p_{n,t}^{\text{ch}} \nonumber \\
&\hspace{3cm}  +c_{n}^\text{dis} p_{n,t}^{\text{dis}}) +\sum_{t\in \mathcal{T}}  \sum_{n\in \mathcal{N}} c_{n}^\text{shed} p_{n,t}^\text{shed} \label{opt-det:operation-obj-2}
\end{align}
\end{subequations}
\fi

The first term $C(\bm{x})$ in the objective represents the annualized investment of storage systems. Cost coefficients for the energy and capacity investments are denoted by $C_{n}^{\text{E}}$ and $C_{n}^{\text{P}}$, which are converted to present values\footnote{Let $\sigma$ be the annual interest and $\Gamma$ be the investment period, e.g. 20 years. $C_{n}^{\text{E}}$ and $C_{n}^{\text{P}}$ are computed as \eqref{eqn:cost-calculation}, where $C_n^{E,\text{total}}$ and $C_n^{P,\text{total}}$ represent the total storage energy and power investment cost over $\Gamma$ years.
\begin{eqnarray}
C_{n}^{\text{E}} = C_{n}^{\text{E},\text{total}} \frac{\sigma (1+\sigma)^\Gamma}{(1+\sigma)^\Gamma-1},~C_{n}^{\text{P}} = C_{n}^{\text{P},\text{total}} \frac{\sigma (1+\sigma)^\Gamma}{(1+\sigma)^\Gamma-1}  \label{eqn:cost-calculation}
\end{eqnarray}
}.
For conceptual simplicity, the second stage uses a typical day to represent the operation of a whole year, i.e. $K_d = 365$. It is straightforward to extend towards employing $D$ typical days to represent the annual operation cost $\sum_{i=1}^{D} K_i c_i(\bm{y})$

\paragraph{Curtailment-Oriented Storage Planning}
Equation \eqref{opt-det:load-curtailment} is the objective function of the curtailment-oriented storage planning formulation, which minimizes total load shedding in the worst-case scenario by investing on storages in the first stage. More specifically, there will be no first-stage cost, i.e., $C(\bm{x})=0$ in  \eqref{opt:det-SP}. The storage planning formulation using \eqref{opt-det:load-curtailment} is termed curtailment-oriented formulation.
\begin{align}
c(\bm{y}) := \sum_{t\in \mathcal{T}}  \sum_{n\in \mathcal{N}}  p_{n,t}^\text{shed}
\label{opt-det:load-curtailment}
\end{align}

\subsubsection{First-stage Constraints} % (fold)
Constraints for the \emph{first stage} $\bm{x} \in \Xi_1$ is defined below:
\begin{equation*}
\Xi_1 := \Big \{ (E_{n}, P_{n}, z_n)\text{s}~\text{that satisfy constraints}~\eqref{discrete-investment:variable}\eqref{opt-det:constr-first-stage}\eqref{opt-det:constr-budget} \Big \}
% \label{opt-det:constraints-stage1}
\end{equation*}
We consider the case where the capacities of storage units are quantized (instead of being continuous), parameters $q^{\text{E}}$ and $q^{\text{P}}$ denote the smallest quantized energy and power capacities for one energy storage unit.  Integer variable $z_n$ is the number of storage units to be installed at bus $n$, which is constrained by the total quantity limit of storage investment \eqref{q_limit}. 
\begin{align}
     z_{n} \in \{0,1,2,\cdots,\overline{z}_{n}\},~n\in \mathcal{N}.  \label{discrete-investment:variable}
\end{align}
As computed in \eqref{energy-discrete} and \eqref{power-discrete}, $E_n$ and $P_n$ represent the energy and power capacities of the storage system at node $n$.
% Constraint \eqref{opt-det:constr-ratio} is the power-capacity ratio constraints on storage units.
\begin{subequations}
\label{opt-det:constr-first-stage}
\begin{align}
& \sum_{n \in \mathcal{N}} z_{n} \le \overline{z} \label{q_limit},\\
& q^{\text{E}} z_{n} = E_{n},~n\in\mathcal{N} \label{energy-discrete},\\
& q^{\text{P}} z_{n} = P_{n},~n\in\mathcal{N} \label{power-discrete}. 
\end{align}
\end{subequations}
Constraint \eqref{opt-det:constr-budget} limits total investment within budget.
\begin{equation}
\sum_{n\in \mathcal{N}} (C_{n}^{\text{E}} E_{n} + C_{n}^{\text{P}} P_{n}) \le C^{\text{budget}} \label{opt-det:constr-budget} 
\end{equation}

\subsubsection{Second-stage Constraints} % (fold)
\label{ssub:second_stage_constraints}
Constraints for the \emph{second stage} $\bm{y} \in \Xi_2(\bm{x}; \bm{\delta})$ are the set of daily operational constraints. Note the feasible region $\Xi_2$ depends on the first-stage decision $\bm{x} = (E_{n}, P_{n})$ and uncertainties $\bm{\delta} = (\alpha^w_{n,t},\alpha^d_{n,t})$.
\ifx\version\arxiv % for arxiv version, single column
\begin{equation}
\Xi_2(E_{n}, P_{n}; \bm{\delta}) := \Big \{(p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}},p_{i,n,t}^{\mathcal{G}},p_{n,t}^\text{shed}, v_{n,t})\text{s}~
\text{that satisfy constraints}~\eqref{opt-det:operation-constraints}  \eqref{opt-det:storage-constraints}\eqref{eqn:not_the_same_time_storage} \Big \}.
% \label{opt-det:constraints-stage2}
\end{equation}
\else
\begin{multline}
\Xi_2(E_{n}, P_{n}; \bm{\delta}) := \Big \{(p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}},p_{i,n,t}^{\mathcal{G}},p_{n,t}^\text{shed}, v_{n,t})\text{s}~\\
\text{that satisfy constraints}~\eqref{opt-det:operation-constraints}  \eqref{opt-det:storage-constraints}\eqref{eqn:not_the_same_time_storage} \Big \}.
% \label{opt-det:constraints-stage2}
\end{multline}
\fi
% \XG{mention $\delta$.}

% % This three-level model allows for "complete recourse", it is a typical two-stage adaptive robust optimization model.
% The planner decides on storage investments about siting and sizing (first level) anticipating the worst uncertainty realization of wind output and load output within an uncertainty set (second level). The operator responses to the variation of daily wind output and load to minimize the worst daily operation cost. Specifically, the objective \eqref{opt-det:obj}) is to minimize the total annual investment and operation costs. The annual operation cost is represented by the worst operation cost not by an average operation cost. Hence, the objective doesn't mean an estimation for real cost, but it is a risk-oriented or safety-oriented formulation which makes the worst operation cost minimized \cite{robust_storage_in}. 

% The constraint \eqref{opt-det:uncertainty set}) represents the considered uncertainty factors within a specific uncertainty set. $\textbf{P}^\text{w}$ and $\textbf{L}^\text{d}$ are vectors representing the daily variation of wind output and load demand in each node of the power system during the target year and are represented by scenarios here.

% For the planning, this scenario-based uncertainty consists of historical data \cite{robust_storage_in} or the scenario generated by designed algorithms. The advantage of the scenario-based uncertainty set is that it can naturally considers the correlation, such as the correlation between wind outputs at different locations or the correlation between loads and wind outputs.  For the lower-level operation problem with "complete recourse",

Constraint \eqref{opt-det:operation-constraints} is about the secure operation of the system, including nodal balance \eqref{opt-det:constr-balance}, generation capacity limits \eqref{opt-det:constr-generation} and ramping limits \eqref{opt-det:constr-ramp}, transmission line flow limits \eqref{opt-det:constr-line}, load shedding limits \eqref{opt-det:constr-cut}, and DC power flow equation \eqref{opt-det:DC-power-flow}. The actual wind output in \eqref{opt-det:operation-constraints} is the product of the maximum wind capacity $\overline{w_{n}}$ at node n and the wind capacity factor $\alpha^w_{n,t}$ at node n at time t. The actual load is the product of the peak load $\overline{d_{n}}$  at node n and the load  factor $\alpha^d_{n,t}$ at node n at time t.
% \begin{subequations}
% \label{opt-det:operation-constraints}
% \begin{align}
% & d_{n,t} = \sum_{i \in \mathcal{G}(n)} p_{i,n,t}^{\mathcal{G}} + p_{n,t}^{\text{dis}} - p_{n,t}^{\text{ch}} + p_{n,t}^{w} + \sum_{j|n\in r(l)} p_{j,t}^{f}   \nonumber \\
% & \hspace{1cm} - \sum_{j|n \in o(l)} p_{j,t}^{f}+ p_{n,t}^{\text{shed}}; \forall n \in \mathcal{N},\forall t \in \mathcal{T} \label{opt-det:constr-balance}  \\
% & \underline{p_i^{\mathcal{G}}} \le p_{i,n,t}^{\mathcal{G}} \le \overline{p_i^{\mathcal{G}}}; \forall i \in \mathcal{G},\forall t \in \mathcal{T} \label{opt-det:constr-generation}\\
% & -\underline{R}_{i} \le p_{i,n,t}^{\mathcal{G}} - p_{i,t-1}^g \le \overline{R}_{i};\forall i \in \mathcal{G},\forall t \in \mathcal{T} \label{opt-det:constr-ramp}\\
% & \underline{p_l^{\mathcal{L}}} \le p_{l,t}^{\mathcal{L}} \le \overline{p_l^{\mathcal{L}}}; \forall j \in \mathcal{L},\forall t \in \mathcal{T}\label{opt-det:constr-line} \\
% & 0 \le p_{n,t}^{\text{shed}} \le d_{n,t}; \forall n \in \mathcal{N},\forall t \in \mathcal{T} \label{opt-det:constr-cut}  \\
% & p_{j,t} = \frac{1}{x_l} (\theta_{o(l),t}-\theta_{r(l),t}); \forall j \in \mathcal{L},\forall t \in \mathcal{T} \label{opt-det:DC-power-flow}
% \end{align}
% \end{subequations}

\ifx\version\arxiv % for arxiv version, single column
\begin{subequations}
\label{opt-det:operation-constraints}
\begin{align}
& \sum_{i \in \mathcal{G}(n)} p_{i,n,t}^{\mathcal{G}} + p_{n,t}^{\text{dis}} - p_{n,t}^{\text{ch}} + \alpha^w_{n,t}\overline{w_{n}} + \sum_{j|n\in r(l)} p_{j,t}^{f} - \sum_{j|n \in o(l)} p_{j,t}^{f}  + p_{n,t}^{\text{shed}} =\alpha^d_{n,t} \overline{d_{n}},\label{opt-det:constr-balance}  \\
& \underline{p_i^{\mathcal{G}}} \le p_{i,n,t}^{\mathcal{G}} \le \overline{p_i^{\mathcal{G}}}, \label{opt-det:constr-generation}\\
& -\underline{R}_{i} \le p_{i,n,t}^{\mathcal{G}} - p_{i,n,t-1}^{\mathcal{G}} \le \overline{R}_{i}, \label{opt-det:constr-ramp}\\
& \underline{p_l^{\mathcal{L}}} \le p_{l,t}^{\mathcal{L}} \le \overline{p_l^{\mathcal{L}}}, \label{opt-det:constr-line} \\
& 0 \le p_{n,t}^{\text{shed}} \le \alpha^d_{n,t}\overline{d_{n}}, \label{opt-det:constr-cut}  \\
& p_{l,t}^{\mathcal{L}} = \frac{1}{x_l} (\theta_{o(l),t}-\theta_{r(l),t}), \label{opt-det:DC-power-flow} \\
& \hspace{2cm} i \in \mathcal{G}(n),~n \in \mathcal{N},~ l \in \mathcal{L},~ t \in \mathcal{T}. \nonumber
\end{align}
\end{subequations}
\else
\begin{subequations}
\label{opt-det:operation-constraints}
\begin{align}
& \sum_{i \in \mathcal{G}(n)} p_{i,n,t}^{\mathcal{G}} + p_{n,t}^{\text{dis}} - p_{n,t}^{\text{ch}} + \alpha^w_{n,t}\overline{w_{n}} + \sum_{j|n\in r(l)} p_{j,t}^{f} - \\
& \hspace{3cm} \sum_{j|n \in o(l)} p_{j,t}^{f}  + p_{n,t}^{\text{shed}} =\alpha^d_{n,t} \overline{d_{n}},\label{opt-det:constr-balance}  \\
& \underline{p_i^{\mathcal{G}}} \le p_{i,n,t}^{\mathcal{G}} \le \overline{p_i^{\mathcal{G}}}, \label{opt-det:constr-generation}\\
& -\underline{R}_{i} \le p_{i,n,t}^{\mathcal{G}} - p_{i,n,t-1}^{\mathcal{G}} \le \overline{R}_{i}, \label{opt-det:constr-ramp}\\
& \underline{p_l^{\mathcal{L}}} \le p_{l,t}^{\mathcal{L}} \le \overline{p_l^{\mathcal{L}}}, \label{opt-det:constr-line} \\
& 0 \le p_{n,t}^{\text{shed}} \le \alpha^d_{n,t}\overline{d_{n}}, \label{opt-det:constr-cut}  \\
& p_{l,t}^{\mathcal{L}} = \frac{1}{x_l} (\theta_{o(l),t}-\theta_{r(l),t}), \label{opt-det:DC-power-flow} \\
& \hspace{2cm} i \in \mathcal{G}(n),~n \in \mathcal{N},~ l \in \mathcal{L},~ t \in \mathcal{T}. \nonumber
\end{align}
\end{subequations}
\fi

Constraints on the energy storage system are in \eqref{opt-det:storage-constraints} and \eqref{eqn:not_the_same_time_storage}, including SOC update from $t-1$ to $t$ in \eqref{opt-det:constr-soc-evolving}, charging and discharging power limits \eqref{opt-det:constr-charging}-\eqref{opt-det:constr-discharging}, and SOC limits \eqref{opt-det:constr-soc}.
% The load shedding variable $p_{n,t}^{d}$ ensures the feasibility of the lower-level operation problem pertaining to any uncertainty realization in \eqref{opt-det:uncertainty set}). It also ensures the relatively complete recourse assumption.
\begin{subequations}
\label{opt-det:storage-constraints}
\begin{align}
& e_{n,t}^{\text{SOC}} - e_{n,t-1}^{\text{SOC}} = p_{n,t}^{\text{ch}}\eta_{n}^{\text{ch}} - p_{n,t}^{\text{dis}}/\eta_{n}^{\text{dis}}, \label{opt-det:constr-soc-evolving} \\
& 0 \le p_{n,t}^{\text{ch}} \le P_{n} \cdot v_{n,t},\label{opt-det:constr-charging} \\
& 0 \le p_{n,t}^{\text{dis}} \le P_{n}\cdot (1-v_{n,t}), \label{opt-det:constr-discharging}  \\
& 0 \le e_{n,t}^{\text{SOC}} \le E_{n},\label{opt-det:constr-soc} \\
& \hspace{3cm} ~n \in \mathcal{N},~t \in \mathcal{T}. \nonumber
\end{align}
\end{subequations}
We introduce binary variables $v_{n,t}$ to avoid charging and discharging at the same time. When $v_{n,t}=1$, the storage system of node $n$ at time $t$ is charging; when $v_{n,t}=0$, the storage system is discharging.
\begin{align}
\label{eqn:not_the_same_time_storage}
v_{n,t} \in \{0,1\},~n \in \mathcal{N},~t \in \mathcal{T}.
\end{align}
% subsection deterministic_{n}torage_planning (end)

\subsection{Robust Storage Planning} % (fold)
\label{sub:robust_storage_planning}
To accurately determine the optimal location and size of energy storage systems, storage planning problems must account for short-term operational uncertainties, as the main benefits of energy storage are smoothing out the fluctuations of renewable generation and facilitating the integration of renewables. 
In the deterministic storage planning model \eqref{opt:det-SP}, wind generation $w_{n,t}=\alpha^w_{n,t}\overline{w_{n}}$ and load $d_{n,t}=\alpha^d_{n,t}\overline{d_{n}}$ are considered as deterministic trajectories. The deterministic approach \eqref{opt:det-SP} fails to take the short-term operational risk into consideration.
In order to accurately quantify the benefits of energy storage with the consideration of operation risk, we propose a two-stage robust storage planning model in this section. By constructing a scenario-based uncertainty set using wind and load data, we show that the operation risk is limited within acceptable ranges.

The proposed two-stage robust storage planning framework is shown in \eqref{opt-robust-compact-nonconvex} .
\begin{align}
\text{(nc-RSP)}:~\min_{ \bm{x} \in \Xi_{1}}~ C(\bm{x}) + K_d \max_{\bm{\delta} \in \Delta} \min_{ \bm{y} \in \Xi_{2}(\bm{x}; \bm{\delta})} c(\bm{y})  \label{opt-robust-compact-nonconvex} 
\end{align}
The uncertainties are modeled by a pre-defined uncertainty set $\Delta$. There is only one difference, i.e., $\max_{\bm{\delta} \in \Delta}$, between the deterministic model \eqref{opt:det-SP} and its robust counterpart \eqref{opt-robust-compact-nonconvex}. By optimizing the decision for the worst-scenario, the solution to \eqref{opt-robust-compact-nonconvex} is immune against all possible realizations of uncertainties in the uncertainty set $\Delta$.

The choice of the uncertainty set $\Delta$ lies at the heart of robust optimization. In this paper, we construct $\Delta = \mathcal{K} = \{\bm{\delta}^{(k)}\}_{k=1}^{|\mathcal{K}|} = \{\{\alpha_{n,t}^{d,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}},\{\alpha_{n,t}^{w,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}}\}_{k=1}^{|\mathcal{K}|}$ using $K$ i.i.d. scenarios $\{\bm{\delta}^{(k)}\}_{k=1}^{|\mathcal{K}|}$. Each operational scenario consists of daily load factor profiles $\{\alpha_{n,t}^{d,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}}$ and daily profiles of renewable capacity factors $\{\alpha_{n,t}^{w,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}}$. Essentially, we use these profiles to depict short-term uncertainties from temporal load variations and renewable fluctuations.  
These operational scenarios could come from historical data \cite{ robust_storage_in} or data-driven scenario generation method \cite{data_scenario}.  One direct benefit of using scenarios is to capture spatial and temporal correlations of uncertainties.   More discussions on the benefits of constructing the scenario-based uncertainty set for storage planning are in Section \ref{sec:theoretical_analysis}. We adopt a relatively simple model of long-term uncertainties. The main long-term uncertainties are presented by the predicted peak load $\overline{d_{n}}$ and renewable capacity $\overline{w_{n}}$, which come from predictions of human experts or state-of-the-art algorithms.
% subsection robust_{n}torage_planning (end)

\subsection{Convex and Non-convex Formulations} % (fold)
\label{sub:convex_and_non_convex_formulations_of_storage_planning}
Due to discrete variables $z_{n,t}$ and $v_{n,t}$, the robust storage planning problem \eqref{opt-robust-compact-nonconvex} is non-convex. To reduce computational burden and obtain better theoretical results, we introduce the convexified version of \eqref{opt-robust-compact-nonconvex} in \eqref{opt-robust-compact-convex}.
We first remove the discrete planning variable $z_{n}$, thus delete constraint \eqref{opt-det:constr-first-stage} and make $P_n$ and $E_n$ main planning decision variables.
\begin{align}
\underline{\rho} E_{n} \le P_{n} \le \overline{\rho} E_{n},~ n\in\mathcal{N}. \label{opt-det:constr-first-stage-relaxed}
\end{align}
\noindent Next we relax the binary variable $v_{n,t}$ (charging/discharging) to continuous variable in \eqref{eqn:relaxed_charging_discharging_no}.
\begin{equation}
\label{eqn:relaxed_charging_discharging_no}
0 \le v_{n,t} \le 1,~n \in \mathcal{N},~t \in \mathcal{T}.
\end{equation}
This relaxation is commonly adopted when studying storage system operations. Several sufficient conditions were derived to guarantee the exactness of this relaxation, and many simulation results reported that this relaxation was exact in most cases, e.g., \cite{storage_sufficient_condition,xu_scalable_2017}.

After the modifications above, we denote the convexified feasible region as $\breve{\Xi}_1$.
\begin{equation*}
\breve{\Xi}_1 := \Big \{ (E_{n}, P_{n}, z_n)\text{s}~\text{that satisfy constraints}~\eqref{opt-det:constr-first-stage}\eqref{opt-det:constr-budget}\eqref{opt-det:constr-first-stage-relaxed} \Big \}
% \label{opt-det:constraints-stage1-convex}
\end{equation*}
The feasible region of the second stage $\breve{\Xi}_2(E_{n}, P_{n}; \bm{\delta})$ is
\ifx\version\arxiv % for arxiv version, single column
\begin{equation*}
\breve{\Xi}_2(E_{n}, P_{n}; \bm{\delta}) := \Big \{(p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}},p_{i,n,t}^{\mathcal{G}},p_{n,t}^\text{shed})\text{s} 
~\text{that satisfy constraints}~\eqref{opt-det:operation-constraints}  \eqref{opt-det:storage-constraints}\eqref{eqn:relaxed_charging_discharging_no} \Big \}.
% \label{opt-det:constraints-stage2-convex}
\end{equation*}
\else
\begin{multline*}
\breve{\Xi}_2(E_{n}, P_{n}; \bm{\delta}) := \Big \{(p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}},p_{i,n,t}^{\mathcal{G}},p_{n,t}^\text{shed})\text{s} \\
~\text{that satisfy constraints}~\eqref{opt-det:operation-constraints}  \eqref{opt-det:storage-constraints}\eqref{eqn:relaxed_charging_discharging_no} \Big \}.
% \label{opt-det:constraints-stage2-convex}
\end{multline*}
\fi

The convexified robust storage planning problem is in \eqref{opt-robust-compact-convex}. Notice that both the first and second stages of (c-RSP) are convex.
\begin{align}
\text{(c-RSP)}:~\min_{ \bm{x} \in \breve{\Xi}_{1}}~ C(\bm{x}) + K_d \max_{\bm{\delta} \in \Delta} \min_{ \bm{y} \in \breve{\Xi}_{2}(\bm{x}; \bm{\delta})} c(\bm{y})  \label{opt-robust-compact-convex} 
\end{align}
In fact, the convex formulation \eqref{opt-robust-compact-convex} is also widely adopted in the storage planning studies, e.g., \cite{storage_sizing_2015,storage_deg_2020}. The convex storage planning model also has two formulations: cost-oriented with objective function \eqref{opt-det:cost} and curtailment-oriented with objective function \eqref{opt-det:load-curtailment}.

In the remainder of this paper, we refer to \eqref{opt-robust-compact-nonconvex} as non-convex robust storage planning (nc-RSP), and \eqref{opt-robust-compact-convex} as convex robust storage planning (c-RSP). 
Both (c-RSP) and (nc-RSP) will be solved using the C\&CG algorithm introduced in Section \ref{sub:column_and_constraint_generation_algorithm}. 
% \begin{align}
% \breve{\Xi}_1 := &\Big \{ (E_{n}, P_{n})\text{s}~\text{that satisfy constraints}~\eqref{opt-det:constr-budget}\eqref{opt-det:constr-ratio} \Big \} \label{opt-det:constraints-stage1-convex}
% \end{align}
% \begin{multline}
% \breve{\Xi}_2(E_{n}, P_{n}; \bm{\delta}) := \Big \{(p_{n,t}^{\text{ch}},p_{n,t}^{\text{dis}},p_{i,n,t}^{\mathcal{G}},p_{n,t}^\text{shed})\text{s} \\
% \text{that satisfy constraints}~\eqref{opt-det:operation-constraints}  \eqref{opt-det:storage-constraints} \Big \}. \label{opt-det:constraints-stage2}
% \end{multline}

Four different formulations are studied in this paper
\begin{table}[htbp]
  \caption{Four different formulations being studied}
  \label{tab:four_formulations}
  \centering

  \begin{tabular}{l|c|c|c|c}
  \hline

  \hline
   & \multicolumn{2}{c|}{\textbf{cost-oriented} } & \multicolumn{2}{c}{\textbf{curtailment-oriented} } \\
  \cline{2-5} 
   & (c-RSP) & (nc-RSP) &  (c-RSP) & (nc-RSP) \\
  \hline
  \textbf{Objective}  & \eqref{opt-det:cost} & \eqref{opt-det:cost} & \eqref{opt-det:load-curtailment} & \eqref{opt-det:load-curtailment} \\
  \hline
  \textbf{1st stage} & \eqref{opt-det:constr-first-stage}\eqref{opt-det:constr-budget}\eqref{opt-det:constr-first-stage-relaxed} & \eqref{discrete-investment:variable}\eqref{opt-det:constr-first-stage}\eqref{opt-det:constr-budget} & \eqref{opt-det:constr-first-stage}\eqref{opt-det:constr-budget}\eqref{opt-det:constr-first-stage-relaxed} & \eqref{discrete-investment:variable}\eqref{opt-det:constr-first-stage}\eqref{opt-det:constr-budget} \\
  \textbf{2nd stage} & \eqref{opt-det:operation-constraints}\eqref{opt-det:storage-constraints}\eqref{eqn:relaxed_charging_discharging_no} & \eqref{opt-det:operation-constraints}\eqref{opt-det:storage-constraints}\eqref{eqn:not_the_same_time_storage} & \eqref{opt-det:operation-constraints}\eqref{opt-det:storage-constraints}\eqref{eqn:relaxed_charging_discharging_no} & \eqref{opt-det:operation-constraints}\eqref{opt-det:storage-constraints}\eqref{eqn:not_the_same_time_storage} \\
  \hline

  \hline
  \end{tabular}
\end{table}

% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_{n}im}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_{n}econd_case}}
%\caption{Simulation results for the network.}
%\label{fig_{n}im}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.

\section{Theoretical Analysis} % (fold)
\label{sec:theoretical_analysis}
The careful choice of uncertainty set $\Delta$ is critical to get meaningful storage planning results. Throughout this paper, we adopt a data-driven approach to constructing uncertainty set $\Delta = \mathcal{K} = \{\bm{\delta}^{(k)}\}_{k=1}^{|\mathcal{K}|} = \{\{\alpha_{n,t}^{d,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}},\{\alpha_{n,t}^{w,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}}\}_{k=1}^{|\mathcal{K}|}$ using $K$ i.i.d. scenarios $\{\bm{\delta}^{(k)}\}_{k=1}^{|\mathcal{K}|}$. 
This simple yet powerful choice of uncertainty set originates from the scenario approach \cite{campi_exact_2008,campi_wait-and-judge_2016,campi_general_2018}. This section demonstrates many advantages of this simple choice of uncertainty set.
Section \ref{sub:basic_properties}  analyzes some basic properties of the scenario-based robust storage planning problem. Sections \ref{sub:theoretical_guarantees_cRSP} and \ref{sub:theoretical_guarantees_ncRSP} investigate the procedures and main benefits of obtaining guarantees.

\subsection{Basic Properties} % (fold)
\label{sub:basic_properties}
\subsubsection{On Relatively Complete Resource} % (fold)
\label{ssub:on_relatively_complete_resource}
\begin{rem}
\label{rem:load_shedding_give_complete_recourse}
When allowing load shedding, both (c-RSP) and (nc-RSP) have relatively complete recourse.
\end{rem}
Note that all theorems in Section \ref{sub:probabilistic_feasibility_guarantees_via_the_scenario_approach} requires the relatively complete recourse assumption. Remark \ref{rem:load_shedding_give_complete_recourse} states that our RSP formulations satisfy this assumption. 
This remark follows common sense of power system operations. When a system is in severe situations, a common control action is to shed load (e.g., rotating outages). Remark \ref{rem:load_shedding_give_complete_recourse} essentially states that we can shed load to a lower level to maintain minimum generation, thus the second stage problem (DCOPF) is feasible at the high cost of load shedding. We also want to point out that Remark \ref{rem:load_shedding_give_complete_recourse} does not hold if the following two types of constraints are added: (1) no load shedding is allowed, i.e., $p_{n,t}^{\text{shed}}=0$; or (2) load shedding is limited, i.e., $\sum_{n \in \mathcal{N}} p_{n,t}^{\text{shed}} \le \overline{p}^{\text{shed}}$.
All results in Sections \ref{sub:theoretical_guarantees_cRSP} and \ref{sub:theoretical_guarantees_ncRSP} are for the cases with load shedding, thus meets the relatively complete recourse assumption. Similar theoretical results are still possible without the relatively complete recourse assumption, e.g., Theorem 4.1 in \cite{calafiore_random_2010}.
% subsection on_relatively_complete_resource (end)

\subsubsection{On Violation Probability} % (fold)
\label{ssub:on_violation_probability}
Similar with Section \ref{sec:background}, we introduce an auxiliary variable $\gamma$ to denote the worst-case cost ($\gamma \ge c(\bm{y})$). Let $(\bm{x}^*, \gamma^*)$ denote the optimal (first-stage) solution to (c-RSP) or (nc-RSP). 
Remark \ref{rem:violation_probability_interpretation_general} explains the meaning of $\mathbb{V}(\bm{x}^*,\gamma^*)$ for general two-stage RO problem. Similarly, in the context of robust storage planning, $\mathbb{V}(\bm{x}^*,\gamma^*)$ also depicts the probability of two events: (1) infeasible second-stage problem (infeasible DCOPF); or (2) there exists a feasible operation, but its objective value $\gamma$ is greater than $\gamma^*$. Detailed interpretation of  $\mathbb{V}(\bm{x}^*,\gamma^*)$ differ in the cost-oriented and curtailment-oriented formulations.

\paragraph{Interpretation of $\mathbb{V}(\bm{x}^*,\gamma^*)$ in Cost-oriented Formulation} % (fold)
\label{par:interpretation_of_in_cost_oriented_formulation}

% paragraph interpretation_of_in_cost_oriented_formulation (end)
% \begin{rem}[Violation Probabilities in the Context of Storage Planning]
% \label{rem:meaning_of_violation_prob}
As stated in Remark \ref{rem:load_shedding_give_complete_recourse}, when allowing load shedding, the second stage is always feasible, thus $\mathbb{V}(\bm{x}^*,\gamma^*)$ only depicts event (2), i.e., the operation cost $\bm{d}^\intercal y(\bm{\delta}; \bm{x}^*)$ is greater than the objective value $\gamma^*$:
\begin{equation}
\label{eqn:violation_prob_in_storage_planning}
\mathbb{V}(\bm{x}^*, \gamma^*) = \mathbb{P}_{\bm{\delta}}\big( \bm{d}^\intercal y(\bm{\delta}; \bm{x}^*) > \gamma^* \big)
\end{equation}
% \end{rem}

\XG{significant revision is neede for the following paragraphs}




\paragraph{Interpretation of $\mathbb{V}(\bm{x}^*,\gamma^*)$ in Curtailment-oriented Formulation} % (fold)
\label{par:interpretation_of_in_cost_oriented_formulation}
For the curtailment-oriented robust planning formulation, $\mathbb{V}(\bm{x}^*, \gamma^*)$ means the risk of the actual load shedding is greater than the curtailment $\gamma^*_{d}$. Of course, in addition to the risk of load shedding, it also can be the risk of renewable curtailment, it is up to the formulation. 

Especially, for the curtailment-oriented formulation, when $\gamma^*=0$, $\mathbb{V}(\bm{x}^*, \gamma^*)$ means the risk of load shedding is greater than 0. This is essentially the loss of load probability (LOLP), which is an important indication for power system reliability. Usually, we can use the following procedure to obtain a planning solution satisfying the reliability requirement, i.e. the daily LOLP within acceptable ranges. 
\begin{enumerate}
\item Execute the computation procedures in part B or part C \XG{what are these?} for (c-RSP) or (nc-RSP) to obtain the solution $\bm{x}^*, \gamma^*$ satisfying the risk guarantee $\epsilon$ (i.e. LOLP).
\item If $\gamma^*=0$, terminate the computation; otherwise, add the investment budget $C^{budget}$ or quantity budget $\overline{z}$ in an increment $\Delta C$ or $\Delta z$ , then go back to step 1). 
\end{enumerate}
Sections \ref{sub:theoretical_guarantees_cRSP} and \ref{sub:theoretical_guarantees_ncRSP} present analysis on the violation probabilities $\mathbb{V}(\bm{x}^*,\gamma^*)$. 
% subsubsection on_the_violation_probability (end)

% \subsubsection{On the Budget Constraint} % (fold)
% \label{ssub:budget_constraint}
% active or inactive budget constraints

% $\sum_{n\in \mathcal{N}} (C_{n}^{\text{E}} E_{n} + C_{n}^{\text{P}} P_{n}) \le C^{\text{budget}}$, \eqref{opt-det:constr-budget}, 
% % subsubsection budget_constraints (end)

\subsection{A-Priori Guarantees for (c-RSP)} % (fold)
\label{sub:theoretical_guarantees_cRSP}
% \begin{prop}
% \label{prop:invariant_set_storage_planning_one}
% The minimal invariant set of (c-RSP) is a singleton ($|\mathcal{I}| = 1$), i.e., the scenario with the largest cost. 
% \end{prop}
% \begin{proof}[Proof of Proposition \ref{prop:invariant_set_storage_planning_one}]
  
% \end{proof}


\begin{cor}[Prior Guarantees for (c-RSP)]
\label{cor:a_priori_guarantee_c_RSP}
Consider the convex RSP formulation (c-RSP) with $|\mathcal{S}|$ candidate storage locations.
Given an acceptable risk level $\epsilon \in (0,1)$ and a confidence parameter $\beta \in (0,1)$. 
Let $(\bm{x}^*, \gamma^*)$ be the optimal solution to (c-RSP) with $K$ i.i.d. scenarios, and $K$ be the smallest integer that
\begin{equation}
\label{eqn:K_choice_c_RSP}
\sum_{i=0}^{2|\mathcal{S}|} \binom{N}{i} \epsilon^i (1- \epsilon)^{N-i} \le \beta.
\end{equation}
then $\mathbb{P}^K\big( \mathbb{V}(\bm{x}_{\mathcal{K}}^*, \gamma^*) > \epsilon \big) \le \beta$.
\end{cor}

% \begin{thm}[A-Priori Guarantees]
% \label{thm:apriori_guarantee_convex}
% Suppose \eqref{opt:two-stage-robust-two-scenario} is convex and has relatively complete recourse, and $(\bm{x}_{\mathcal{K}}^*, \gamma^*)$ is the optimal solution to \eqref{opt:two-stage-robust-two-scenario}, then the following probabilistic guarantee holds:
% \begin{equation}
% \mathbb{P}^K\big( \mathbb{V}(\bm{x}_{\mathcal{K}}^*, \gamma^*) > \epsilon \big) \le \sum_{i=0}^{1} \binom{K}{i} \epsilon^i (1- \epsilon)^{K-i}.
% \end{equation}
% \end{thm}

For the large-scale system, where many candidate storage locations $\mathcal{S}$ are being considered, Corollary \ref{cor:a_priori_guarantee_c_RSP} might lead to a large-scale optimization problem including astronomical scenarios, which is inefficient to solve. In Section \ref{sec:case_study}, after solving  hundreds of instances of (c-RSP) on different systems, we found that the essential set of every instance of (c-RSP) always had cardinality one, i.e., $|\mathcal{I}|=1$. This feature of $|\mathcal{I}|=1$ is very appealing, as it holds for any problem size or system scale. \XG{this is not rigorous, need modification.}
Because of this observation, we can significantly improve the results of Corollary \ref{cor:a_priori_guarantee_c_RSP} using Theorem \ref{thm:aposteriori_guarantee_convex}.

% Based on that, we can apply Theorem \ref{thm:aposteriori_guarantee_convex} to the large-scale (c-RSP) by fisrt making an assumption $|\mathcal{I}|=1$, then  verifying if the assumption is true. 

% The main procedures to solve (c-RSP) and obtain probabilistic guarantees are summarized below:
% % This feature of $|\mathcal{I}|=1$ is very appealing, as it holds for any problem size or system scale. If it is always true for (c-RSP), the theoretical guarantees and sample complexity $K$ 

% \begin{enumerate}
% \item choose acceptable risk level $\epsilon$ and confidence parameter $\beta$, assume the cardinality of invariant set $|\mathcal{I}| = 1$;
% \item compute the smallest integer $K$ satisfying $\epsilon(|\mathcal{I}|,\beta) \ge \epsilon$ using \eqref{eqn:poster_convex_epsilon_function};
% \item construct uncertainty set $\Delta$ using $K$ i.i.d. scenarios $\mathcal{K} = \{\bm{\delta}^{(k)}\}_{k=1}^{K}$;
% \item solve (c-RSP) with $\Delta = \mathcal{K}$ using C\&CG algorithm, which returns the optimal storage planning solution $(\bm{x}^*, \gamma^*)$ and an invariant set $\mathcal{O}$;
% \item  compute the irreducible (or essential) invariant set $\mathcal{I}_{\mathcal{K}}$ based on Algorithm \ref{alg:irr};
% \item compute the posterior risk level $\epsilon(|\mathcal{I}_{\mathcal{K}}|)$ using \eqref{eqn:poster_convex_epsilon_function}.
% \item If $\epsilon(|\mathcal{I}_{\mathcal{K}}|)$ $\leq$ $\epsilon$, output the result; otherwise, go to step 2) with $|\mathcal{I}| =|\mathcal{I}_{\mathcal{K}}|$.
% \end{enumerate}

\subsection{A-Posterior Guarantees} % (fold)
\label{sub:theoretical_guarantees_ncRSP}
\subsubsection{On Invariant Sets} % (fold)
\label{ssub:on_invariant_sets}
According to Proposition \ref{prop:CCG_return_invariant_set}, invariant sets of the scenario-based robust storage planning (RSP) model can be directly obtained after the C\&CG algorithm converges. Then a greedy algorithm (see Algorithm \ref{alg:irr} in Appendix \ref{sub:algorithms}) can further pinpoint the essential set. Since the C\&CG algorithm usually converges within a few iterations, the obtained invariant set is often small. This is an attractive computational feature since Algorithm \ref{alg:irr} will stop within a few iterations as well. Algorithm \ref{alg:irr} can be applied to btoh (c-RSP) and (nc-RSP).

The minor computational burden of finding the essential set for (c-RSP) and (nc-RSP) makes it possible to obtain a-posteriori guarantees for the planning solutions via Theorems \ref{thm:aposteriori_guarantee_convex} and \ref{thm:aposteriori_guarantee_nonconvex}. Specifically, we design the algorithms in part B and part C for (c-RSP) and (nc-RSP) through verifying the cardinality of invariant set fast to provide the posterior risk guarantees. \XG{what does part B and C mean?}

\begin{prop}
\label{prop:invariant_set_convex}
The invariant set of (c-RSP) has cardinality no more than $2|\mathcal{S}|+1$, where $\mathcal{S}$ denotes the set of candidate locations for storage planning.
\end{prop}

\begin{rem}
Since (c-RSP) is convex, Theorem \ref{thm:number_of_support_scenarios_convex_case} can be directly applied. The cardinality of the invariant set of (c-RSP) is bounded by the total number of decision variables (both first and second stages), which is significantly larger than $2|\mathcal{S}|+1$. Proposition \ref{prop:invariant_set_convex} significantly tightens the upper bound and reduces the scenario requirement in Theorems \ref{thm:apriori_guarantee_convex}, \ref{thm:aposteriori_guarantee_convex} and \ref{thm:aposteriori_guarantee_nonconvex}. For example, in the 118-bus system, there are $|\mathcal{S}|=??$ \XG{tell me a number} candidate locations, and xxxx decision variable in total.
\end{rem}
In our numerical simulations, we surprisingly found that the invariant set of (c-RSP) is often a singleton, i.e., $|\mathcal{I}| = 1$. Since the sample complexity requirement in Theorems \ref{thm:apriori_guarantee_convex}, \ref{thm:aposteriori_guarantee_convex} and \ref{thm:aposteriori_guarantee_nonconvex} grow monotonically with $|\mathcal{I}|$. The case of $|\mathcal{I}| = 1$ is the best non-trivial case, in the sense that it requires the least amount of scenarios to achieve an acceptable risk level $\epsilon$. Furthermore, Proposition \ref{prop:invariant_set_convex} is independent of system size, which implies that the proposed approach will not require too many scenarios when applying on large-scale real-world systems.

\ifx\version\arxiv
One first attempt to explain the reason that $|\mathcal{I}|=1$ for (c-RSP) is Proposition \ref{prop:invariant_set_singleton}, which improves Proposition \ref{prop:invariant_set_convex} for special cases.
% Using the same technique (see Theorem \ref{thm:equivalent_RLP_formulations}) of proving Proposition \ref{prop:two-stage-RO-as-one-stage}, we can show that \eqref{opt:two-stage-robust-single} is equivalent with the following maximin problem
% \begin{align}
% \max_{\bm{\delta} \in \Delta} ~ \min_{\bm{x} \in \mathcal{X}}~&\bm{c}^{\intercal} \bm{x} + \gamma \\
% \text{s.t.}~&  (\bm{x},\gamma) \in \mathcal{Z}(\bm{\delta}) 
% \end{align}
\begin{defn}[Worst Scenario]
\label{defn:worst_scenario}
The \emph{worst scenario} of \eqref{opt:two-stage-robust} is defined as $\bm{\delta}^* := \arg \max_{\bm{\delta} \in \Delta} f(\bm{\delta})$, where $f(\bm{\delta}) := \min_{\bm{x} \in \mathcal{X}, (\bm{x},\gamma) \in \mathcal{Z}(\bm{\delta}) } \bm{c}^{\intercal} \bm{x} + \gamma$.
% The set of worst scenarios is denoted by $\Omega$.
\end{defn}
% For general choices of uncertainty set $\Delta$, the worst scenario may not be unique, $\Omega$ may not even be a finite set.
% \begin{prop}
% Under Assumption \ref{def:relative} (relatively complete recourse), the essential set $\mathcal{E}$ of \eqref{opt:two-stage-robust-scenarios} has cardinality no more than 1, $|\mathcal{E}| \le 1$. \XG{Main proof idea is based on the relatively complete recourse assumption, it does not change the domain of $f(\bm{\delta})$, but I'm still doubting the if the maximin problem is truely equivalent with the original two-stage formulation, the key question here is $Z(\bm{\delta})$ is still constraint-wise uncertainty.} \XG{therefore I chose to present a much weaker version below, which I feel confident about its correctness.}
% \end{prop}
\begin{prop}
\label{prop:invariant_set_singleton}
If the worst scenario $\bm{\delta}^*$ of \eqref{opt:two-stage-robust-scenarios} is unique, then $\mathcal{I} = \Omega = \{\bm{\delta}^*\}$, thus $|\mathcal{I}|=1$.
\end{prop}
Although Proposition \ref{prop:invariant_set_singleton} holds correct for non-convex problems as well, the main issue here is that we need to find the global optimal solution. Table \ref{Tab:support scenario} provides an example that suboptimal solution leads to more than one elements in the invariant set.
\fi

In general, it is challenging to obtain a-priori guarantees for non-convex problems. The only known result is Theorem \ref{thm:aposteriori_guarantee_nonconvex}, which provides a-posteriori guarantees. From hundreds of (nc-RSP) instances we solved, most of them have $|\mathcal{I}| \le 2$. The feature makes the application of Theorem \ref{thm:aposteriori_guarantee_nonconvex} for large-scale (nc-RSP) possible.  Even though a-priori guarantees for (nc-RSP) are not possible, we can first compute the sample complexity $K$ based on a guess on $|\mathcal{I}|$ , after solving (nc-RSP),  verifying if this initial guess is correct. The main procedures to solve (nc-RSP) and obtain a-posteriori guarantees based on Theorem \ref{thm:aposteriori_guarantee_nonconvex} are summarized in Algorithm \ref{alg:procedures_to_get_guarantees}.

% \begin{cor}[Probabilistic Guarantees for (nc-RSP)]
% \label{cor:a_posteriori_guarantee_nc_RSP}
% Let the solution be  $(\bm{x}_{\mathcal{K}}^*, \gamma^*)$ optimal solution, let $|\mathcal{I}|$ be the cardinality of the invariant set, then the following probabilistic guarantee holds:
% \begin{equation}
% \mathbb{P}^K\big( \mathbb{V}(\bm{x}_{\mathcal{K}}^*, \gamma^*) > \epsilon(|\mathcal{I}_{\mathcal{K}}|, \beta) \big) \le \beta,
% \end{equation}
% \begin{equation}
% \label{eqn:sample_complexity_nc_RSP}
% \text{and}~\epsilon(k,\beta) := 
%   \begin{cases}
%   1&~\text{if}~k=K \\
%   1 - \Big( \frac{\beta}{N \binom{N}{k}} \Big)^{\frac{1}{N-k}} &~\text{otherwise}.
%   \end{cases}
% \end{equation}
% \end{cor}

% For (nc-RSP), Corollary \ref{cor:a_posteriori_guarantee_nc_RSP} provides a-posteriori risk guarantee. Note the cardinality of the invariant  set of nc-RSP is unknown before the computation. Therefore, the following algorithm is designed for nc-RSP through assuming the cardinality of its invariant set in advance.
% \begin{algorithm}
%  \caption{Storage Planning with Discrete Investment Variables}
%    \label{alg:planning_discret}
%  \begin{algorithmic}[1]
%  \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%  \renewcommand{\algorithmicensure}{\textbf{Output:}}
%  \REQUIRE $\epsilon$, $\beta$, $s_{K}^*=1$, $K$,  $M$, $\epsilon({s_{K}^*)}=+\infty$.
%  %\ENSURE  out
%  \\ \textit{Independent Planning Experiments} :
%   \FOR {m=1 to M}
%  \WHILE {$\epsilon({s_{K}^*)}>\epsilon$}
%   \STATE {Numerically find a $K$ satisfying $\epsilon({s_{K}^*)}$ $\le$   $\epsilon$ by \eqref{thm:non-convex-scenario-2}.}
%   \STATE {Generate $K$ independent scenarios to construct the uncertainty set;}
%   \STATE {Solve the robust planning model \eqref{opt-robust-compact} with discrete investment constraints \eqref{opt-robust: discrete-investment});}
%   \STATE {Find the cardinality of the irreducible set $s_{K}^*$ by \textbf{Algorithm 1}. }
%   \STATE {calculate $\epsilon({s_{K}^*)}$ Use \eqref{thm:non-convex-scenario-2} in  \textbf{Theorem 3} to ; }
%   \ENDWHILE
%   \ENDFOR
%   \STATE {Find the solution $\bm{x}^*$ with the minimum investment cost from the $M$ planning solutions \{$\bm{x}_1,\cdots,\bm{x}_M$\}. }
%  \RETURN { $\bm{x}^*$  }
%  \end{algorithmic} 
%  \end{algorithm}
% \XG{make it an algorithm}
% \begin{enumerate}
% \item choose acceptable risk level $\epsilon$ and confidence parameter $\beta$, assume the cardinality of invariant set $|\mathcal{I}| = 1$;
% \item compute the smallest integer $K$ satisfying $\epsilon(|\mathcal{I}|,\beta) \ge \epsilon$ using \eqref{eqn:sample_complexity_nonconvex_epsilon}  
% ;
% \item construct uncertainty set $\Delta$ using $K$ i.i.d. scenarios $\mathcal{K} = \{\bm{\delta}^{(k)}\}_{k=1}^{K}$;
% \item solve (nc-RSP) with $\Delta = \mathcal{K}$ using C\&CG algorithm, which returns the optimal storage planning solution $(\bm{x}^*, \gamma^*)$ and an invariant set $\mathcal{O}$;
% \item  compute the irreducible (or essential) invariant set $\mathcal{I}_{\mathcal{K}}$ based on Algorithm \ref{alg:irr};
% \item compute the posterior risk level $\epsilon(|\mathcal{I}_{\mathcal{K}}|)$ using \eqref{eqn:sample_complexity_nonconvex_epsilon}.
% \item If $\epsilon(|\mathcal{I}_{\mathcal{K}}|)$ $\leq$ $\epsilon$, output the result; otherwise, go to step 2) with $|\mathcal{I}| =|\mathcal{I}_{\mathcal{K}}|$.
% \end{enumerate}

\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE Choose acceptable risk level $\epsilon$ and confidence parameter $\beta$;
\STATE Guess the cardinality of invariant set $|\mathcal{I}| \leftarrow k$;
\STATE Compute the smallest integer $K$ satisfying $\epsilon(|\mathcal{I}|,\beta) \ge \epsilon$; use \eqref{eqn:poster_convex_epsilon_function} in Theorem \ref{thm:aposteriori_guarantee_convex} when solving (c-RSP); use \eqref{eqn:sample_complexity_nonconvex_epsilon} in Theorem \ref{thm:aposteriori_guarantee_nonconvex}when solving (nc-RSP);
\STATE Construct uncertainty set using $K$ i.i.d. scenarios $\mathcal{K} \leftarrow \{\bm{\delta}^{(k)}\}_{k=1}^{K}$;
\STATE Solve the RSP problem with uncertainty set $\mathcal{K}$ using C\&CG algorithm, obtain the optimal storage planning solution $(\bm{x}^*, \gamma^*)$ and an invariant set $\mathcal{O}$;
\STATE Compute the irreducible (or essential) invariant set $\mathcal{I}_{\mathcal{K}} \subseteq \mathcal{O}$ using Algorithm \ref{alg:irr};
\IF {$|\mathcal{I}_{\mathcal{K}}| > k$}
\STATE Go to step 2 with $k \leftarrow |\mathcal{I}_{\mathcal{K}}|$;
\ELSE 
\STATE Output the optimal solution $(\bm{x}^*, \gamma^*)$, uncertainty set $\mathcal{K}$, invariant set $|\mathcal{I}_{\mathcal{K}}|$, and theoretical guarantee $\mathbb{P}^{K}(\mathbb{V}(\bm{x}^*, \gamma^*) \le \epsilon) \ge 1 - \beta$.
\ENDIF
% \STATE otherwise, 
% \STATE compute the posterior risk level $\epsilon(|\mathcal{I}_{\mathcal{K}}|)$ using \eqref{eqn:sample_complexity_nonconvex_epsilon}.
\end{algorithmic}
\caption{Obtaining Theoretical Guarantees for RSP Solutions}
\label{alg:procedures_to_get_guarantees}
\end{algorithm}


% subsection theoretical_guarantees_for_ (end)

\subsection{Reduce Conservativeness and Find Better Solutions} % (fold)
\label{sub:improve_solution_quality}
The procedures described in Sections \ref{sub:theoretical_guarantees_cRSP} and \ref{sub:theoretical_guarantees_ncRSP} are essentially a randomized algorithm. More specifically, solutions to (c-RSP) or (nc-RSP) with different sets of scenarios of the same size $K$ could be different, but all of them possess the same theoretical guarantees as in Sections \ref{sub:theoretical_guarantees_cRSP} and \ref{sub:theoretical_guarantees_ncRSP}. We can exploit the randomness of the algorithm to get better storage planning decisions and reduce conservativeness. For example, in Section \ref{sec:case_study}, we solved (c-RSP) or (nc-RSP) 10 times using 10 different datasets of the same size, then chose the storage planning solutions with the least investment cost. By doing this, we avoided some overly conservative solutions due to drawing extreme random samples.


% The theory can guarantee the solution can be against the future risk of short-term operation uncertainty, which maybe from the varying mode of renewable and load.  	
% We can obtain a least investment cost solution with the same risk guarantee and the similar total operational cost. Due to the randomized properties, the investment solutions from the planning experiments with the same sample complexity but different random scenarios are usually different. They would have the same risk guarantees, meanwhile, these robust planning solutions usually have very close actual operational cost. These good properties allow us to choose a least-cost investment among the multiple random planning experiments. A more rigorous analysis is possible via order statistics, which beyond the scope of this paper. 



% \begin{prop}
% Reduce conservativeness. 
% \begin{equation}
% (1 - \beta)^M \approx 1 - M \beta
% \end{equation}
% but the randomness is reduced.
% \end{prop}


\section{Case Study} % (fold)
\label{sec:case_study}
Two case studies are presented in this section. The first case study investigates the performance of the proposed approach in an environment with \emph{abundant data}. The uncertainties are depicted using probability distributions, from which we can sample as many scenarios as we need. The second case study is a thorough investigation of the proposed approach in a more realistic setting, i.e., a real-life-size large-scale system with a only moderate number of scenarios. We generate the scenarios for planning totally based on the historical operational data. 
% In both cases, we examine the proposed approach in the following aspects: (1) convex versus non-convex formulations; (2) solutions with different number of scenarios; (3) quality of the optimal solution. risk level versus sample complexity; (3) .
% In both cases, the proposed approach worked well and the theoretical guarantees hold regardless of the modeling of uncertainties. 
Both case studies share the same settings of energy storage systems, critical parameters are summarized in Table \ref{tab:parameters}.
\begin{table*}[tb]
  \caption{Critical Parameters of Energy Storage Systems}
  \label{tab:parameters}
  \centering

  \begin{tabular}{l|ccccccccccc}
  \hline

  \hline
  Parameter & $C_{n}^{\text{P}}$ & $C_{n}^{\text{E}}$ & $\Gamma$ & $\sigma$ & $\eta_{n}^{\text{ch}}, \eta_{n}^{\text{dis}}$ & $\overline{\rho}, \underline{\rho}$ & $K_d$ & $c_{n}^{\text{dis}}, c_{n}^{\text{ch}}$ & $q^{\text{E}}$ & $q^{\text{P}}$ & $\overline{z}$, $\overline{z}_n$\\
  \hline
  Value & $500$\$/kW & $20$\$/kWh & $10$ Years & $10\%$ & $0.9$,~$0.9$ & $0.8$, $0.2$ & $365$ & $18$\$/MW, $1$\$/MW & $32$MWh & $8$MW & $20$, $4$ \\
  \hline

  \hline
  \end{tabular}
\end{table*}

Since the scenario approach is a \emph{randomized} algorithm\cite{campi_exact_2008}, it is necessary to quantify the randomness of the solution returned by the scenario approach. Specifically, for a given sample complexity $N$, we repetitively solved RSP using 10 independent sets of $N$ scenarios. Each one of those 10 problems solved is referred as \emph{an experiment} in this section.

\subsection{IEEE 6-bus system}
\label{sub:ieee_6bus_case_study}
\subsubsection{System configuration} % (fold)
% \label{ssub:system_configuration}
The first case study is based on a modified IEEE 6-bus system \cite{data_driven_planning}. We added two 100MW wind farms at buses 5 and 6, and increased the cost coefficients of coal and natural gas plants 20\% higher than the original case. Key parameters of storage investment are in Table \ref{tab:parameters}.
% In this case study, the convex model is mainly used.

The uncertainties of load and wind are modeled by probability distributions. We first generated wind speed data from Weibull distributions\footnote{Key parameters: scale factor $11.0086$m/s, shape factor $1.9622$m/s, cut-in speed $V_\text{ci}=4$m/s, rated speed $V_\text{rated}=13.61$m/s, $V_\text{co}=25$m/s).}. The output of wind farms was computed based on the generated wind speed data using equation (44) in \cite{robust_storage_in}.
The load scenarios were generated by adding generated forecast errors on 365 days of historic load profiles in \cite{robust_storage_in}. We assume the load forecast errors follow a Gaussian distribution $\mathcal{N}(0,1\%)$. 
% subsubsection system_configuration (end)

\subsubsection{Planning Results with Different Risk Guarantee Parameter $\epsilon$}
\label{ssub:6bus_results_diff_epsilon}
 In  this case, we study the impact of sample complexity $N$ on the robust planning solution considering the randomness of the algorithm. We examine the costs and variances of 10 solutions of 10 experiments at the same sample complexity, i.e. the same risk level. There are 6 candidate locations in the test system, i.e. $|\mathcal{S}|=6$. When adopting the prior risk guarantees, i.e. Theorem \ref{thm:apriori_guarantee_convex},
given different risk parameters $\epsilon$, we computed the sample complexity $K$ with the same confidence parameter $\beta=10^{-3}$ in the Corollary \ref{cor:a_priori_guarantee_c_RSP}  . Results are in Table \ref{tab:priori_sample_complexity_convexity}. Given $K$ i.i.d. scenarios, we solved (c-RSP) and obtained optimal storage planning decisions. 
% \ref{fig:performance}.
\begin{table}[htbp]
  \caption{The sample complexity for the different a-priori risk guarantees, using Theorem }
  \centering
  \begin{tabular}{l|cccccc}
  \hline

  \hline
  \textbf{A-priori risk level $\epsilon$} & \textbf{5\%} & \textbf{10\%} & \textbf{20\%} & \textbf{30\%} & \textbf{40\%} & \textbf{50\%} \\
  \hline
  \textbf{Sample complexity $K$}   & 796 & 398 & 199 & 133 & 100 & 80\\
  \hline

  \hline
  \end{tabular}
  \label{tab:priori_sample_complexity_convexity}
\end{table}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{6-bus-5.pdf}
  \caption{Storage Planning Results with Different A-priori Risk Guarantees $\epsilon$. All results were computed based on 10 independent experiments (Section \ref{ssub:6bus_results_diff_epsilon}).}
  \label{fig:multi}
\end{figure}

The first row of Fig. \ref{fig:multi} shows two components in the objective of (r-RSP): investment cost $C(\bm{x})$ and worst-case operational cost $c(\bm{y})$. Clearly planning decisions of larger risk parameters $\epsilon$ require less planning investments.
Although the top-right panel of Fig. \ref{fig:multi} also shows worst-case operational cost $c(\bm{y})$ decreases with increasing risk parameters $\epsilon$, we would like to emphasize that the worst-case operational cost $c(\bm{y})$ of (c-RSP) was evaluated on the sampled $K$ scenarios, which \emph{does not represent true operational costs}.

The true operational cost was estimated using another independent $1.6\times 10^4$ test scenarios, it is shown as the ``out-of-sample'' operation cost $c(\bm{y})$ in the bottom-right panel of Fig. \ref{fig:multi}. Clearly, the true operation cost increases with risk parameters $\epsilon$, since more load shedding will arise.
The optimal solution $\gamma^*$ of (r-RSP) provides an estimate of worst-case operation cost. The bottom-left figure of Fig. \ref{fig:multi} shows $\mathbb{V}(\bm{x}^*, \gamma^*)$, i.e., the probability that the true operation cost is higher than $\gamma^*$ (see Remark \ref{rem:violation_probability_interpretation_general} and Section \ref{ssub:on_violation_probability}
). 

The second row of Fig. \ref{fig:multi} examines the randomness in the planning decisions. The main metric being used here is the coefficient of variance (COV), which is defined by the ratio of standard deviation of a random variable to its mean. Fig. \ref{fig:multi} illustrates the positive correlation between $\epsilon$ and COV values, more risk-averse (smaller $\epsilon$) solutions are more stable (smaller COV). "WPC" means the worst-case operation cost.

\subsubsection{Planning Results with Different Investment Budgets $C^{\text{budget}}$} % (fold)
\label{ssub:results_with_varying_investment_budgets}
Results of 10 experiments with the the same risk guarantee parameters ($\epsilon=0.01$, $\beta=10^{-3}$, $K=920$) but varying budgets $C^{\text{budget}}$ are presented below.
% The robust storage planning problem is essentially seeking a balance between current investment and future savings in operation.
We take a closer look at these two interesting cases in the following subsections. The case studies adopt the posterior risk guarantee for \emph{c-RSP} and correspond to Theorem \ref{thm:aposteriori_guarantee_convex} and the computation procedures in Section \ref{sub:theoretical_guarantees_cRSP}. For each result of planning experiment, we compute its out-of-sample risk level through sampling another $1.6*10^4$ scenarios from the uncertainty distribution as test data.  

\paragraph{Adequate Investment Budget ($C(\bm{x}^*) < C^{\text{budget}}$)} % (fold)
\label{par:inactive_budget_constraints}
When the investment budget is adequate, i.e., inactive budget constraint $C(\bm{x}^*) < C^{\text{budget}} = \$6 \times 10^6$, the storage installment will \emph{eliminate} load shedding in all scenarios in the uncertainty set $\mathcal{K}$.
Planning results are reported in Fig. \ref{fig:6-bus-a-priori-risk} show the storage investment costs and out-of-sample operation cost risk levels of all planning experiments. The cardinality of Invariant Set of all planning experiments are found to be 1. Since the out-of-sample violation probabilities (risk levels) are all below the risk parameter $\epsilon=0.01$ (red dotted line), we can choose the planning result with the lowest cost. This could effectively reduce the randomness and conservativeness of the scenario approach.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{6-bus-1.pdf}
  \caption{Storage planning results with adequate investment budget ($C(\bm{x}^*) < C^{\text{budget}}$)}
  \label{fig:6-bus-a-priori-risk}
\end{figure}

Despite that the storage planning decisions of 10 experiments have different investment costs, they would not lead to the different actual operation cost. Actual operation cost is represented by the \emph{average} value of the operation costs of $1.6*10^4$ out-of-sample test scenarios.   The \emph{average} operation cost are almost identical, as shown in the bottom-left panel of Fig. \ref{fig:performance}. Hence, in the first row of Fig. \ref{fig:performance}, the investment costs and the total out-of-sample costs of the 10 experiments have the nearly same variation trend and amplitude. However, the bottom-right panel of Fig. \ref{fig:performance} shows that the worst-case operation cost in (c-RSP) varies due to drawing extreme scenarios. It is worth noting that the worst-case operation cost, instead of the \emph{average} operation cost, is embedded in the robust storage planning model. It is a good choice to avoid risks, but it  cannot reflect the actual operation costs. Our method can trade-off the cost and risk in the robust planning model.

% the blue circles represent the investment costs, the two black solid lines indicate the amplitude of variation of investment costs among the 10  independent planning experiments. The red circles represent the out-of-sample total system costs which show the same changing shape as that of the investment costs. The two black solid lines indicate the range of out-of-sample system operational costs among the 10 independent planning experiments. 
\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{6-bus-2.pdf}
\caption{Investment cost and operation costs with adequate investment budget ($C(\bm{x}^*) < C^{\text{budget}}$)}
\label{fig:performance}
\end{figure}

% In the second row of Fig. \ref{fig:performance}, we focus on the operational costs. The left shows the average operational costs of the 10 planning experiments are nearly the same, the right shows the different worst-case operational costs of the 10 planning experiments. Because in the real-life operation, there is a very low chance to meet the worst-case operational scenario, most scenarios are common scenarios. For those most common scenarios, they do not need the same amount of storage investment as the worst-case operational scenario does to improve the system operational cost, and their operational costs under different storage investments are nearly the same. That is the reason for their average operational costs are nearly the same. This also explains why the differences in costs of the 10 planning experiments are mainly on the investment costs, their system operational costs have very minor impacts.

% paragraph inactive_budget_constraints (end)

\paragraph{Inadequate Investment Budget $C(\bm{x}^*) = C^{\text{budget}}$} % (fold)
\label{par:active_budget_constraints}
% \XG{come back to this after revising the theoretical section.}
When the budget is inadequate, the budget constraint is active $C(\bm{x}^*) = C^{\text{budget}}$, load shedding are necessary in extreme scenarios. To ensure the load shedding risk of the planning solution, we resort to the curtailment-oriented formulation. In the first row  of Fig. \ref{fig:storage-incressing-investment-6} , the investment budget is gradually increased and the load shedding is decreased to zero. According to the above theoretical analysis,  the investment solution at $2.4\times10^6\$$ (0 load shedding) can provide the needed load shedding risk guarantee 0.01. 
Even though, at the investment $1.8\times10^6\$$, the out-of-sample load shedding risk requirement seems to be satisfied.  Considering the randomized property of the planning solutions, we adopt the planning solution in the investment of $2.4\times10^6\$$. Besides, all operation cost risks have been satisfied shown in the second row. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{6-bus-4.pdf}
  \caption{Storage planning with gradual increasing investments. }
  \label{fig:storage-incressing-investment-6}
\end{figure}
% paragraph active_budget_constraints (end)
% subsubsection results_with_varying_investment_budgets (end)

\subsection{IEEE 118-bus system}
\subsubsection{System Configuration} % (fold)
\label{ssub:system_configuration}
We conducted numerical simulations on a modified 118-bus system\footnote{The original system is available at \url{http://motor.ece.iit.edu/data}.
% this is for arXiV version
Additional changes include generation costs are set 20\% higher than the original case. The hourly ramp rates of generators are set to 45\% of the maximum generation for the largest units in the system.} with five 200MW wind farms added to buses 16, 37, 48, 75 and 83. All 118 buses are candidate sites for storage installation. The wind and load profiles are from the Electric Reliability Council of Texas (ERCOT)\footnote{Historical load data of ERCOT is from \url{http://www.ercot.com/mktinfo/loadprofile/alp}. Wind data is from \url{http://www.ercot.com/gridinfo/resource}.}.
The dataset consists of about 7300 days (20 years) of hourly wind and load profiles.
It is worth noting that we converted the wind generation profiles to wind capacity factor $\{\alpha_{n,t}^{w,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}}$ ($0\sim 100\%$ of full capacities).
Load profiles were converted to load factors $\{\alpha_{n,t}^{d,(k)}\}_{n \in \mathcal{N}, t \in \mathcal{T}}$ ($0\sim 100\%$) using annual peak loads.
We would like to emphasize that the wind factors depict short-term variations of wind speed, and load factors model the temporal patterns. We scaled the wind and load factors up according to the predicted peak loads and wind capacities of the modified 118-bus system.
%\XG{Talk to Chao to figure out what he means for the sentences below:} Note the peak load and wind capacity at each node maybe change with time, we can not directly use the historical data as the input data. But we think the varying mode of uncertain data at each bus is not variable with the capacity. For example, the varying mode is the temporal wind output capacity factor (i.e. the rate of hourly output to capacity at a bus) or the temporal load factor (i.e. the rate of hourly load to peak load at a bus). They represent the short-term uncertainty in the planning problem.
%For example, Fig. \ref{fig:varying mode} shows 10 daily wind output and load varying mode, they are from the ECORT's historic data. However, the change of peak load and wind capacity at each node is the long-term uncertainty. In this paper, they are considered have been given by experts or professional prediction methods. Therefore, we extract the different varying modes of wind output and load from the historical output data of each year in the 20-year data set as the data set. Then by multiplying them with the predicted peak load and wind capacity, we can obtain the final data set. . These historical data are rescaled to meet the peak load and wind farm capacity settings of the 118-bus system. Fig. \ref{fig:varying mode} plots the \emph{normalized} load and wind profiles of 10 days from ERCOT historical data.
\ifx\version\arxiv
Wind capacity factors and load factors of 10 consecutive days are plotted in Figure \ref{fig:varying mode}.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{varying_mode.pdf}
  \centering
  \caption{10 Daily profiles of load factor and wind capacity factor in ECORT historical data}
  \label{fig:varying mode}
\end{figure}
\fi

\subsubsection{Storage Planning Results of Four Different Formulations} % (fold)
\label{ssub:storage_planning_results_of_four_different_formulations}
Similar to the 6-bus case in Section \ref{sub:ieee_6bus_case_study}, 10 experiments on the 118-bus system were conducted.
In each experiment, the 7300-day dataset was divided into two non-overlapping subsets.
The first subset contained 5000 days and served as the test dataset to evaluate out-of-sample results. The second subset consisted all remaining scenarios, which is used as input to the scenario approach. Storage planning results using four different formulations (see Table \ref{tab:four_formulations}) are reported in Figure \ref{fig:118-bus-results}. In all experiments, we used the same parameters $\epsilon=0.01$ and $\beta=0.001$. For non-convex formulations (nc-RSP), we used different parameters $\overline{z}_n = 10$ and $\overline{z}=1000$ from Table \ref{tab:parameters}.
\XG{say something about different approaches to obtain theoretical guarantees. using different } All results were obtained using the procedures in Section xxx.
% The first subset was the random sampled scenarios from the data set as input to (c-RSP) or (nc-RSP), the second part is the 5000 daily scenarios in the remaining data, which served as the test dataset to compute out-of-sample results. Actually, if we adopt more than 3000 scenarios as input to (c-RSP) or (nc-RSP), the remaining 4000 scenarios will be used as test data set.
\begin{figure*}[tb]
\begin{subfigure}[t]{0.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{non-convex-cost.pdf}
  \caption{Cost-oriented (c-RSP).}
  \label{fig:118-bus-continuous-investments-cost}
\end{subfigure}
\begin{subfigure}[t]{0.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{convex-cost.pdf}
  \caption{Cost-oriented (nc-RSP)}
  \label{fig:118-bus-discrete-investments-cost}
\end{subfigure}
\begin{subfigure}[t]{0.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{convex-load.pdf}
  \caption{Curtailment-oriented (c-RSP)}
  \label{fig:118-bus-continuous-investments-load}
\end{subfigure}
\begin{subfigure}[t]{0.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{non-convex-load.pdf}
  \caption{Curtailment-oriented (nc-RSP)}
  \label{fig:118-bus-discrete-investments-load}
\end{subfigure}
\caption{Storage planning Results of the IEEE 118-bus system, using four different formulations in Table \ref{tab:four_formulations}}
\label{fig:118-bus-results}
\end{figure*}

\paragraph{Using Cost-oriented Formulation} 
Fig. \ref{fig:118-bus-continuous-investments-cost} shows the storage planning results with adequate investment budget $C(\bm{x}) < C^{\text{budget}}=\$12\times10^7$.
% Each planning experiment employed the historical data being sampled randomly from the historical data. Then the other 5000 historical data is used to calculate the out-of-sample risk level to verify the risk guarantee.
No experiment reached the investment budget $C^{\text{budget}} $ and all experiments successfully maintained out-of-sample risk $\hat{\epsilon}$ within acceptable ranges ($\hat{\epsilon} < 0.01$). The largest out-of-sample risk level $\hat{\epsilon}=0.0068 \le 0.01$ happened in the $10^{th}$ planning experiment. This verifies the probabilistic guarantees in Theorem \ref{thm:aposteriori_guarantee_convex}.

% The results mean when we use the other historical data to verify the planning result, the theoretical guarantee is still hold. We could select the planning decision with the smallest investment cost to reduce conservativeness, this is similar to Section \ref{par:inactive_budget_constraints}.
%688
%The bottom row of Fig. \ref{fig:118-bus-continuous investments} shows the results of active budget constraint $C(\bm{x}) = C^{\text{budget}}$. All ten experiments reach investment budget $C^{\text{budget}} = 1.2\times10^6\$$ to reduce cost of load shedding. As shown in Fig. \ref{fig:storage-incressing-investment-6} and \ref{fig:118-bus-continuous investments}, by repetitively solving RSP problems with different parameters (such as $C^{\text{budget}}$, $\epsilon$ and $K$), we can find out the best solution that balances investment budget and operational risk. \YC{Of course, we also can find a planning solution with operational constraints risk guarantee through adjusting $C^{budget}$ in the safety-based robust planning model}

%Assume the number of support scenarios is 1, the number of input scenarios ranges from 100 to 1200,  Fig. \ref{fig:post-bound} shows that these two posterior probability bounds for convex(blue) and non-convex(orange) decision problems show the difference.   
%\begin{figure}[htbp]
  %\centering
  %\includegraphics[width=\linewidth]{post-bound.pdf}
  %\centering
  %\caption{A-posterior probability bounds for convex and non-convex decision problems; \XG{including the convex priori guarantee, need to use Chao's code} \YC{add a line, a-priori guarantee, using num of support scenario=1} }
 % \label{fig:post-bound}
%\end{figure}
Figure \ref{fig:118-bus-discrete-investments-cost} is the case that employs the non-convex storage planning model (nc-RSP), in which the capacities of energy storages are quantized. The y-axis in Figure \ref{fig:118-bus-discrete-investments-cost} is the total number of energy storage units to be installed.
We started to by assuming $|\mathcal{I}|=1$ based on our observations after solving hundreds of (c-RSP) and (nc-RSP), and computed $K=2250$ using \XG{eq} to guarantee $\epsilon=0.01$ and $\beta=0.001$.
The out-of-sample violation probabilities in all 10 experiments are smaller than $\epsilon=0.01$, this verifies Theorem \ref{thm:aposteriori_guarantee_nonconvex}. Notice that the smallest total investment in storage units happened at the $9$th experiment, in which the largest out-of-sample $\hat{\epsilon} = 0.0078 < 0.01$ is within acceptable ranges. 
% The maximum investment quantity is 220 units ($2^{th}$ experiment), the minimum investment quantity is 157 units ($9^{th}$ experiment).
\ifx\version\arxiv
Notice that the $1$st and $10$th experiments have the same total storage units, this does not indicate the same storage planning solution, since they can be installed in different locations.
\fi

\paragraph{Using Curtailment-oriented Formulation} 
Fig. \ref{fig:118-bus-continuous-investments-load} shows the convex planning result pursuing the posterior load-curtailment risk guarantee by the curtailment-oriented formulation. To better study the impact of investment on load shedding, in this case, the peak load level is 1.2 times of that in the above cost-oriented planing experiment. With the increase of the investment budget, at the investment of $6 \times 10^7\$$, the out-of-sample risk level $\hat{\epsilon}$ is approaching the load shedding risk requirement $\epsilon = 0.01$.  But considering the randomized property of the planning solution, the planning solution at the investment of $8 \times 10^7\$$ should be employed because of the 0 load shedding is reached. The blue star is the objective function of the curtailment-oriented formulation, i.e. the maximum load shedding. The 0-curtailment means the risk requirement $\epsilon = 0.01$ is ensured according to the above theoretical analysis. The out-of-sample risk level (green line) based on historical data also verified the risk guarantee.


When the investment quantity is limited, the load-curtailment risk is important. Fig. \ref{fig:118-bus-continuous-investments-load} shows the non-convex planning result pursuing the posterior load-curtailment risk guarantee by the curtailment-oriented formulation. This experiment corresponds to the above curtailment-oriented convex planning experiment, their peak load levels and other system parameters are the same. With the increase of the investment quantity, at the investment of 150 units, the out-of-sample risk level $\hat{\epsilon}$ is below the load shedding risk requirement $\epsilon$ 0.01. The theoretical guarantee is hold at 225 units. The blue star indicates that the objective of the curtailment-oriented model reaches 0 at 225 units.
When we compared the non-convex and convex planning results by converting the quantity to investment cost, it is easy to find that the non-convex planning model needs more cost to reach the needed load shedding risk guarantee. That is because the investment of quantized storage units have more physical limitations than the continuous storage units.
% paragraph cost_oriented_formulation_versus_curtailment_oriented_formulation (end)

\subsubsection{Convex Formulation versus Non-convex Formulation} % (fold)
\label{ssub:convex_formulation_versus_non_convex_formulation}
\begin{itemize}
\item Convex formulations essential set always has cardinality 1
\item Non-convex formulations, sometimes 1, but not always which is not true, always no greater than 3, Table \ref{Tab:support scenario} gives one example.
\end{itemize}
Although this is a much bigger system, we observed that the cardinality of essential sets is still always $1$. The same risk level can be achieved with the same amount of scenarios as the 6-bus case. Namely, with $\epsilon=0.01$ and $\beta=10^{-3}$, the 118-bus system requires the same number of scenarios $K=920$ as the 6-bus system. 

\XG{In practice, we can use all available scenarios to obtain more risk-averse (i.e., smaller $\epsilon$) solutions, without reserving a major part of datasets for out-of-sample analysis. This allows us to fully exploit the value of limited data, which is one major advantage of having theoretical guarantees. }

After solving (nc-RSP) using the C\&CG algorithm, we found that the cardinality of invariant sets in all 10 experiments were $1$, thus we stopped here. However, we would like to point out that $|\mathcal{I}|$ could be more than 1 when solving . We were able to create a case with $|\mathcal{I}|=2$
% subsubsection convex_formulation_versus_non_convex_formulation (end)

\subsubsection{Obtaining Theoretical Guarantees} % (fold)
\label{ssub:finding_essential_set}
We illustrate the process of searching for essential set $\mathcal{E}$ and obtaining theoretical guarantees using one instance of (nc-RSP). 
Based on our experiences in Section \ref{ssub:convex_formulation_versus_non_convex_formulation}, we first assume $|\mathcal{E}| = 1$. Given $\epsilon=$ and $\beta=$, we computed $K=2220$ using equation \XG{equation}. 
We first solved (nc-RSP) with $2220$ scenarios via C\&CG algorithm. Besides the optimal storage planning solution and optimal objective value $2.4253\times 10^9 \$$, C\&CG algorithm also returned an invariant set $\mathcal{I} = \{589, 164, 1732\}$ (Proposition \ref{prop:CCG_return_invariant_set}). 
Algorithm \ref{alg:irr} started with $\mathcal{I} = \{589, 164, 1732\}$ and removes scnearios one by one to check if the invariant set can be furture reduced.
Table \ref{Tab:support scenario} illustrates this process.
\begin{table}[htbp]
  \caption{Finding Essential Set for (nc-RSP)}
  \label{Tab:support scenario}
  \centering

  \begin{tabular}{r|cccc}
  \hline

  \hline
  \textbf{Iter} & \textbf{Scenario} & \textbf{Invariant Set} & \textbf{Objective Value} & \textbf{Invariant Set} \\
  \textbf{No.} &  \textbf{Removed} & \textbf{After Removal} & \textbf{After Removal} & \textbf{Updated} \\
  % & \textbf{to be Removed} & \textbf{$\mathcal{I} -s$ After Removal} & \\
  \hline
  0   & -  & \{164,  589, 1732\} & \$$2.4253\times 10^9$ & \{164, 589, 1732\} \\
  1   & 164 &  \{589, 1732\} & \$$2.4253 \times 10^9$  & \{589, 1732\} \\
  2   & 589 & \{1732\} &  \$$2.2765 \times 10^9$ & \{589, 1732\} \\
  3   & 1732  & \{589\} &  \$$2.3224 \times 10^9$ & \{589, 1732\} \\
  \hline

  \hline
  \end{tabular}
\end{table}
The first row of Table \ref{Tab:support scenario} shows the initialization of Algorithm \ref{alg:irr}. In the first iteration, scenario $164$ was removed and the optimal objective values remained unchanged, thus the updated invariant set is $\{589, 1732\}$. In the second and third iterations, removing scenario $589$ and $1732$ changed optimal solutions, therefore the invariant set $\{589, 1732\}$ cannot be further reduced.

However, notice that the invariant set $\mathcal{I} = \{589, 1732\}$ has cardinality $2$, which is greater than our initial guess $1$.
There are two possibilities of following steps. First, we can stop here if the relaxed guarantee $\epsilon(2) = $ is acceptable. 
The second choice is to recompute $K=3012$ using $\epsilon=$, $\beta=$ and $|\mathcal{I}|=2$, solve (nc-RSP) using another independent set of $3012$ scenarios, and check if the cardinality of the new invariant set is smaller than $2$.


\subsection{Improve Sample Complexity} % (fold)
\label{sub:reducing_sample_complexity}
The sample complexity can be further removed by exploting For example, if from the structure of the
problem it was proved that 
then 
I
according to \emph{Remark 4} in \cite{campi_general_2018}, the equation (9) in \cite{campi_general_2018} can be used to improve the sample complexity in \eqref{non-convex-number}. For the cardinality of Invariant Set being 1, the sample complexity of scenarios will be 1410; for the cardinality of Invariant Set being 2, the sample complexity of scenarios will be 2147. The experiments show when we adopt the improved sample complexity to do the \emph{nc-RSP}, the theoretical risk guarantee is still hold.



% The Fig. \ref{fig:storage-discrete-result}  presents the storage investment results, where and how many storage units should be invested on the 118 buses. The planning result reaches the quantity limit, the out-of-sample operational cost risk is 0.0015, which is below the guarantee 0.01. As for the operational constraints risk guarantee, it can be obtained by algorithm 3. The difference is that we need to adjust the investment quantity limit.

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.9\linewidth]{storage_investment_result.pdf}
%   \centering
%   \caption{Discrete storage planning results  }
%   \label{fig:storage-discrete-result}
% \end{figure}
% \section{Discussions} % (fold)
% \label{sec:discussions}
% \subsection{A comparison between continuous investment variables and discrete investment variables}
% To compare the effect of storage investment with continuous and discrete investment variables, we execute the two planning experiments under similar condition settings. Specifically, the risk guarantees and other parameters are the same. But the total quantity limit for the panning with discrete variables is adjusted to 50. Then for the planning with continuous investment variables, we set an equivalent investment budget constraint on investment cost. Because in the discrete investment, the size of each storage unit is fixed at 32 MWh and 8 MW, in the continuous investment, the ratio of power to capacity is fixed at 0.25. The results in the upper part of Fig. \ref{fig:storage-comparison} show that the continuous investment are distributed on more 19 buses, the discrete investments are only distributed on 15 buses. They invest on the same 11 buses. When we eliminate the investment quantity or budget constraints, the results in the lower part of Fig. \ref{fig:storage-comparison} show similar results. The continuous investments are distributed on 24 buses the discrete investments are on 15. There are the same 14 buses in total. On the other hand, their results also show the difference on the sizes. It means for the same risk guarantee, it is infeasible to do the continuous investment instead of the discrete investment for the storage planning with physical limitations on the size of storage devices.
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=\linewidth]{comparison.pdf}
%   \centering
%   \caption{Storage planning results with continuous and discrete investment variables \XG{Difference between top and bottom figures? Energy versus power capacities?} }
%   \label{fig:storage-comparison}
% \end{figure}
% \XG{if you round up/down the continuous decision variable, the original guarantees do not hold. Then what is the point of these theoretical guarantees. Can we do better than this?}
% After solving \eqref{opt-robust-compact-convex}, if the optimal solution $E_{n}^*$ and $P_{n}^*$ are close to zero, i.e., $E_{n} \approx 0$ and $P_{n} \approx 0$, then the energy storage system will not be installed at bus $n$.The investment for some storage facilities can be regarded as continuous investment variables as stated in \cite{xu_scalable_2017}.

% \subsection{Alternative Formulations} % (fold)
% \label{sub:alternative_formulations}
% \subsubsection{Cost-based Robust Storage Planning} % (fold)
% \label{sub:storage_planning}


% Another formulation \eqref{opt-robust-2:robust-storage-planning} replaces the original objective function in the \eqref{opt-det} with the total load shedding \eqref{opt-robust-2:obj}. This model aims at minimizing the load shedding in the worst operational case.
% \begin{align}
% \min_{ \bm{x} \in \Xi_{1}} \max_{\bm{\delta} \in \Delta} \min_{ \bm{y} \in \Xi_{2}(\bm{x}; \bm{\delta})} \sum_{t\in \mathcal{T}}  \sum_{n\in \mathcal{N}}~&p_{n,t}^\text{shed} \label{opt-robust-2:robust-storage-planning}
% \end{align}

% \subsubsection{The relationship between two robust planning formulations}
% It is easily understandable that when the cost of load shedding $c^{\text{shed}}_n \rightarrow +\infty $, the objective of cost-based robust planning model is the same as that of safety-based robust planning model, i.e. minimizing the load sheddings. Further, considering the operational cost risk and the operational constraints risk, the following \textbf{Corollary 1} illustrates how the cost-based robust planning model can guarantee the two risks at the same time. Its proof is put in APPENDIX A.

% \begin{cor}[The relationship between two robust planning models]
% Considering the cost of load shedding $c^{\text{shed}}_n \rightarrow +\infty $ and there not exist load shedding in all optimized scenarios in the cost-based robust planning  model \eqref{opt-det}, then its solution $x^*$ maintains the operational cost and constraints risk guarantees,  $\text{Risk}_{\text{constraints}} \le \text{Risk}_{\text{cost}} \le \epsilon$.
% \end{cor}
% % subsection alternative_formulations (end)
% % section discussions (end)

\section{Concluding Remarks} % (fold)
\label{sec:concluding_remarks} 
This paper formulates and solves the two-stage robust storage planning problem. We connect the two-stage RO optimization with the scenario approach theory through adopting a scenario-based uncertainty set. This approach can consider a wide range of temporal operational conditions representing the short-term uncertainties and flexibility requirements, and provide theoretical guarantees on the operation risk of optimal storage planning solution. We show that the operation risk consists of two critical components: the risk of exceeding the estimated cost and the risk of load shedding. The theoretical guarantees hold for both non-convex and convex RSP models, and we also demonstrate the methods to tighten the theoretical guarantees. The RSP problem is solved via column and constraint generation algorithm. We also connect the C\&CG algorithm with the scenario approach, and show that C\&CG algorithm is an efficient algorithm to find invariant sets, which is essential to the theoretical guarantees on operation risk. Numerical results on the 6-bus and 118-bus systems verify the correctness of theoretical results.

The proposed scenario-based approach has advantages: due to the structure of the two-stage robust optimization formulation, the invariant set is small and can be found easily. This observation is regardless of the system size, which makes the proposed approach scalable for practical applications. Furthermore, this approach can be easily extended towards more general power system planning problems. It is feasible to consider the planning of generation, transmission and renewable energy in the approach, which is a critical part of our future works.

% \YC{procedures of the storage planning}
% \YC{1. doing the cost-based algorithm, if there are no load shedding in the model, then the result has the operational cost and operational constraints risk at the same time;}
% \YC{2. if there is one load shedding event in these scenarios, then do the safety-based model to guarantee the operational constraints risk}
% \YC{This is the correct procedure of doing the planning, but because the space limit, I think we don't need to express the entire procedures}

% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%

% \newpage
